Capturing Opportunity Costs of Batteries with a Staircase Supply-Demand Function

In the global pursuit of carbon neutrality, the role of batteries is indispensable. They provide pivotal flexibilities to counter uncertainties from renewables, preferably by participating in electricity markets. Unlike thermal generators, however, the dominant type of cost for batteries is opportunity cost, which is more vague and challenging to represent through bids in stipulated formats. This article shows the opposite yet surprising results: The demand-supply function of an ideal battery, considering its opportunity cost, is a staircase function with no more than five segments, which is a perfect match with existing rules in many real electricity markets. The demand-supply function shifts horizontally with price forecasts and vertically with the initial SOC. These results can be generalized to imperfect batteries and numerous battery-like resources, including battery clusters, air-conditioners, and electric vehicle charging stations, although the number of segments may vary. These results pave the way for batteries to participate in electricity markets.

==> BackgroundRef.tex <==
carbon emission goal and electricity has highest ratio:
1. https://www.mckinsey.com/capabilities/sustainability/our-insights/the-net-zero-transition-what-it-would-cost-what-it-could-bring

2. https://www.nationalacademies.org/our-work/accelerating-decarbonization-in-the-united-states-technology-policy-and-societal-dimensions#sectionProjectScope






cabon emission and goal among multiple countries:
1. https://www.visualcapitalist.com/sp/race-to-net-zero-carbon-neutral-goals-by-country/

2. Whitehouse, “President Biden Sets 2030 Greenhouse Gas Pollution Reduction Target,” [online] available at (2021/11/04) https://www.whitehouse.gov/briefing-room/statements-releases/2021/04/22/fact-sheet-president-biden-sets-2030-greenhouse-gas-pollution-reduction-target-aimed-at-creating-good-paying-union-jobs-and-securing-u-s-leadership-on-clean-energy-technologies/. 

3. Progress Report of 
China’s National Carbon Market  https://www.mee.gov.cn/ywdt/xwfb/202407/t20240722\_1082192.shtml



renewable among multiple countries:
1. China Dialogue, “China can benefit from a more ambitious 2030 solar and wind target,” [online] available at (2021/11/04) https://chinadialogue.net/en/energy/china-can-benefit-from-a-more-ambitious-2030-solar-and-wind-target/ 

2. European Environment Agency, “Share of energy consumption from renewable sources in Europe,” [online] available at (2021/11/04) https://www.eea.europa.eu/data-and-maps/indicators/renewable-gross-final-energy-consumption-6/assessment. 

3. %国际可再生能源机构的 2024年可再生能源统计报告
https://www.irena.org/Publications/2024/Jul/Renewable-energy-statistics-2024

uncertainty challenge and renewable curtailment:
1. https://www.eia.gov/todayinenergy/detail.php?id=60822
2. https://www.reuters.com/business/energy/rising-curtailments-texas-magnify-grid-storage-shortfalls-2023-10-19/
3. https://www.sciencedirect.com/science/article/pii/S2542435121002440
4. https://www.eia.gov/todayinenergy/detail.php?id=60822






energy storage trends:
1. U.S. Energy Storage Monitor, “U.S. Energy Storage Monitor”,[online] available at  https://www.woodmac.com/industry/power-and-renewables/us-energy-storage-monitor/.
2. https://www.lazard.com/media/42dnsswd/lazards-levelized-cost-of-storage-version-70-vf.pdf


battery optimal actions profile:
1. https://hornsdalepowerreserve.com.au/live-data-graph/
2. 

==> Introduction_v0.tex <==
\par As an urgent and indispensable measure to achieving a sustainable world, the goal of carbon neutrality has become a global consensus. Power generation is the largest source of carbon emission by sector globally\cite{nationalacademies,mckinsey}. In China, which is the country with the largest amount of carbon emission, it accounts for more than 40\% \cite{Chinaecologyandenvironment}. Thus the transition from fossil-fuelled power generation to renewable energy sources (RES) is a paramount mission in our efforts towards a carbon-neutral and sustainable society.

We have indeed seen rapid development in renewable energy in recent years. The International Energy Agency (IEA) projects a substantial increase in global renewable energy capacity, expected to reach approximately 7,300 gigawatts (GW) by 2028—an expansion nearly 2.5 times the current capacity. By 2025, renewables are expected to overtake coal, emerging as the largest source of global electricity generation. \cite{iearenewables}. Well-developed renewable energy systems can significantly reduce carbon footprints, support global climate goals \cite{verpoort2024impact}, and lead to long-term economic benefits including lower energy costs and reduced vulnerability to fossil fuel price volatility \cite{rode2021estimating}. %(Cite some paper about recent development, Nature one, path study ...)

However, unlike thermal units, wind turbines and photovoltaic panels do not have reservoirs of primary energy. Handling uncertainties and volatility of RESs while maintaining a reliable power supply to consumers has been the most significant challenge to our power and energy systems nowadays \cite{millstein2021solar, USeia}. At high penetration levels, there can be times when wind and solar generation exceeds the grid’s capacity to use or store the energy, leading to curtailment. \textcolor{blue}{For instance, as PV penetration increases, curtailment rates rise, particularly in systems with limited flexibility. At lower penetration levels (around 20\%), curtailment is minimal, but it escalates significantly between 25\% and 40\%, potentially exceeding 50\% in high PV scenarios without adequate management of generation variability \cite{huang2024potential}. This undermines the economic viability of renewables \cite{heptonstall2021systematic}.}

Batteries are one of the best measures to tackle these challenges. We see rapid development, cost reduction, and new types of batteries. \textcolor{blue} {Large-scale participation of batteries can shave peak load, reduce the intermittency of renewable energy, increase the efficiency of power use, and provide fast-ramping and high-quality regulation services \cite{wang2023accelerating}. For short-term storage (up to 12 hours), lithium-ion batteries and pumped hydropower storage (PHS) are cost-effective and efficient. By 2040, energy consumption in lithium-ion battery production is expected to decrease by 62–71\%, depending on cell chemistry \cite{degen2023energy}. Mid-duration needs are best served by vanadium redox flow batteries (VRBs), which balance cost and performance. For long-duration storage (beyond 36 hours), hydrogen storage, particularly with geologic storage, and natural gas with carbon capture (NG-CCS) are the most viable, offering significant cost reductions \cite{hunter2021techno}. In systems where renewables supply 60–90\% of electricity, LDES is critical, potentially reducing system costs by up to 50\% when energy capacity costs drop below \$20/kWh \cite{sepulveda2021design, dowling2020role}.} %Moreover, the management techniques of batteries are developed to address the inherent degradation that impacts both operational decisions and economic viability \cite{he2018intertemporal}. }


As more batteries are deployed in the electric power system, they should naturally become active participants in the electricity market, similar to other types of resources \cite{livedatagraph}. Given their charging and discharging capabilities, batteries may bid a demand-supply function, representing their willingness to buy or sell at different prices. In the ideal case, we expect batteries to bid truthfully, bidding their supply-demand functions according to their costs.\par As an urgent and indispensable measure to achieving a sustainable world, the goal of carbon neutrality has become a global consensus. Power generation is the largest source of carbon emission by sector globally\cite{nationalacademies,mckinsey}. In China, which is the country with the largest amount of carbon emission, it accounts for more than 40\% \cite{Chinaecologyandenvironment}. Thus the transition from fossil-fuelled power generation to renewable energy sources (RES) is a paramount mission in our efforts towards a carbon-neutral and sustainable society.

We have indeed seen rapid development in renewable energy in recent years. The International Energy Agency (IEA) projects a substantial increase in global renewable energy capacity, expected to reach approximately 7,300 gigawatts (GW) by 2028—an expansion nearly 2.5 times the current capacity. By 2025, renewables are expected to overtake coal, emerging as the largest source of global electricity generation. \cite{iearenewables}. Well-developed renewable energy systems can significantly reduce carbon footprints, support global climate goals \cite{verpoort2024impact}, and lead to long-term economic benefits including lower energy costs and reduced vulnerability to fossil fuel price volatility \cite{rode2021estimating}. %(Cite some paper about recent development, Nature one, path study ...)

However, unlike thermal units, wind turbines and photovoltaic panels do not have reservoirs of primary energy. Handling uncertainties and volatility of RESs while maintaining a reliable power supply to consumers has been the most significant challenge to our power and energy systems nowadays \cite{millstein2021solar, USeia}. At high penetration levels, there can be times when wind and solar generation exceeds the grid’s capacity to use or store the energy, leading to curtailment. \textcolor{blue}{For instance, as PV penetration increases, curtailment rates rise, particularly in systems with limited flexibility. At lower penetration levels (around 20\%), curtailment is minimal, but it escalates significantly between 25\% and 40\%, potentially exceeding 50\% in high PV scenarios without adequate management of generation variability \cite{huang2024potential}. This undermines the economic viability of renewables \cite{heptonstall2021systematic}.}

Batteries are one of the best measures to tackle these challenges. We see rapid development, cost reduction, and new types of batteries. \textcolor{blue} {Large-scale participation of batteries can shave peak load, reduce the intermittency of renewable energy, increase the efficiency of power use, and provide fast-ramping and high-quality regulation services \cite{wang2023accelerating}. For short-term storage (up to 12 hours), lithium-ion batteries and pumped hydropower storage (PHS) are cost-effective and efficient. By 2040, energy consumption in lithium-ion battery production is expected to decrease by 62–71\%, depending on cell chemistry \cite{degen2023energy}. Mid-duration needs are best served by vanadium redox flow batteries (VRBs), which balance cost and performance. For long-duration storage (beyond 36 hours), hydrogen storage, particularly with geologic storage, and natural gas with carbon capture (NG-CCS) are the most viable, offering significant cost reductions \cite{hunter2021techno}. In systems where renewables supply 60–90\% of electricity, LDES is critical, potentially reducing system costs by up to 50\% when energy capacity costs drop below \$20/kWh \cite{sepulveda2021design, dowling2020role}.} %Moreover, the management techniques of batteries are developed to address the inherent degradation that impacts both operational decisions and economic viability \cite{he2018intertemporal}. }


As more batteries are deployed in the electric power system, they should naturally become active participants in the electricity market, similar to other types of resources \cite{livedatagraph}. Given their charging and discharging capabilities, batteries may bid a demand-supply function, representing their willingness to buy or sell at different prices. In the ideal case, we expect batteries to bid truthfully, bidding their supply-demand functions according to their costs.

==> Introduction_v0_1.tex <==
\par As an urgent and indispensable measure to achieving a sustainable world, the goal of carbon neutrality has become a global consensus. Power generation is the largest source of carbon emission by sector globally \cite{nationalacademies,mckinsey}. In China, which is the country with the largest amount of carbon emission, it accounts for more than 40\% \cite{Chinaecologyandenvironment}. Thus the transition from fossil-fuelled power generation to renewable energy sources (RES) is a paramount mission in our efforts towards a carbon-neutral and sustainable society.

We have indeed seen rapid development in renewable energy in recent years. The International Energy Agency (IEA) projects a substantial increase in global renewable energy capacity, expected to reach approximately 7,300 gigawatts (GW) by 2028—an expansion nearly 2.5 times the current capacity. By 2025, renewables are expected to overtake coal, emerging as the largest source of global electricity generation \cite{iearenewables}. Well-developed renewable energy systems can significantly reduce carbon footprints, support global climate goals \cite{verpoort2024impact}, and lead to long-term economic benefits including lower energy costs and reduced vulnerability to fossil fuel price volatility \cite{rode2021estimating}. %(Cite some paper about recent development, Nature one, path study ...)

However, unlike thermal units, wind turbines and photovoltaic (PV) panels do not have reservoirs of primary energy. Handling uncertainties and volatility of RESs while maintaining a reliable power supply to consumers has been the most significant challenge to our power and energy systems nowadays \cite{millstein2021solar, USeia}. At high penetration levels, there can be times when wind and solar generation exceeds the grid’s capacity to use or store the energy, leading to curtailment. For instance, as PV penetration increases, curtailment rates rise, potentially exceeding 50\% in high PV penetration scenarios without adequate management of generation variability \cite{frew2021curtailment}. This undermines the economic viability of renewables \cite{heptonstall2021systematic}.

Batteries are one of the best measures to tackle these challenges. We see rapid development, cost reduction, and new types of batteries. For short-term storage (up to 12 hours), lithium-ion batteries and pumped hydropower storage (PHS) are cost-effective and efficient. By 2040, energy consumption in lithium-ion battery production is expected to decrease by 62–71\%, depending on cell chemistry \cite{degen2023energy}. Mid-duration needs are best served by vanadium redox flow batteries (VRBs), which balance cost and performance. For long-duration storage (beyond 36 hours), hydrogen storage, particularly with geologic storage, and natural gas with carbon capture (NG-CCS) are the most viable, offering significant cost reductions \cite{hunter2021techno}. In systems where renewables supply 60–90\% of electricity, LDES is critical, potentially reducing system costs by up to 50\% when energy capacity costs drop below \$20/kWh \cite{sepulveda2021design, dowling2020role}. Economic and mature technologies enable large-scale integrations of batteries in power systems, supporting peak load shaving, renewable intermittency reduction, and high-quality regulation services with their fast charging/discharging abilities \cite{wang2023accelerating}. %Moreover, the management techniques of batteries are developed to address the inherent degradation that impacts both operational decisions and economic viability \cite{he2018intertemporal}. }


As more batteries are deployed in the electric power system, they should naturally become active participants in the electricity market, similar to other types of resources \cite{livedatagraph}. \textcolor{red}{add citation FERC storage should participate in the market.} Given their charging and discharging capabilities, batteries may bid a demand-supply function, representing their willingness to buy or sell at different prices. In the ideal case, we expect batteries to bid truthfully, bidding their supply-demand functions according to their costs. 


==> Introduction_v0_2.tex <==
\par As an urgent and indispensable measure to achieving a sustainable world, the goal of carbon neutrality has become a global consensus. Power generation is the largest source of carbon emission by sector globally \cite{nationalacademies,mckinsey}. In China, which is the country with the largest amount of carbon emission, it accounts for more than 40\% \cite{Chinaecologyandenvironment}. Thus the transition from fossil-fuelled power generation to renewable energy sources (RES) is a paramount mission in our efforts towards a carbon-neutral and sustainable society.

We have indeed seen rapid development in renewable energy in recent years. The International Energy Agency (IEA) projects a substantial increase in global renewable energy capacity, expected to reach approximately 7,300 gigawatts (GW) by 2028—an expansion nearly 2.5 times the current capacity. By 2025, renewables are expected to overtake coal, emerging as the largest source of global electricity generation \cite{iearenewables}. Well-developed renewable energy systems can significantly reduce carbon footprints, support global climate goals \cite{verpoort2024impact}, and lead to long-term economic benefits including lower energy costs and reduced vulnerability to fossil fuel price volatility \cite{rode2021estimating}. %(Cite some paper about recent development, Nature one, path study ...)

However, unlike thermal units, wind turbines and photovoltaic (PV) panels do not have reservoirs of primary energy. Handling uncertainties and volatility of RESs while maintaining a reliable power supply to consumers has been the most significant challenge to our power and energy systems nowadays \cite{millstein2021solar, USeia}. At high penetration levels, there can be times when wind and solar generation exceeds the grid’s electricity demands capacity to use or store the energy, leading to curtailment. For instance, as PV penetration increases, curtailment rates rise, potentially exceeding 50\% in high PV penetration scenarios without adequate management of generation variability \cite{frew2021curtailment}. This undermines the economic viability of renewables \cite{heptonstall2021systematic}.

Batteries are one of the best measures to tackle these challenges. We see rapid development, cost reduction, and new types of batteries. For short-term storage (up to 12 hours), lithium-ion batteries and pumped hydropower storage (PHS) are cost-effective and efficient. By 2040, energy consumption in lithium-ion battery production is expected to decrease by 62–71\%, depending on cell chemistry \cite{degen2023energy}. Mid-duration needs are best served by vanadium redox flow batteries (VRBs), which balance cost and performance. For long-duration storage (beyond 36 hours), hydrogen storage, particularly with geologic storage, and natural gas with carbon capture (NG-CCS) are the most viable, offering significant cost reductions \cite{hunter2021techno}. In systems where renewables supply 60–90\% of electricity, LDES is critical, potentially reducing system costs by up to 50\% when energy capacity costs drop below \$20/kWh \cite{sepulveda2021design, dowling2020role}. Economic and mature technologies enable large-scale integrations of batteries in power systems, supporting peak load shaving, renewable intermittency reduction, and high-quality regulation services with their fast charging/discharging abilities \cite{wang2023accelerating}. %Moreover, the management techniques of batteries are developed to address the inherent degradation that impacts both operational decisions and economic viability \cite{he2018intertemporal}. }


As more batteries are deployed in the electric power system, they should naturally become active participants in the electricity market, similar to other types of resources \cite{ferc}. Given their charging and discharging capabilities, batteries may bid a demand-supply function, representing their willingness to buy or sell at different prices. In the ideal case, we expect batteries to bid truthfully, bidding their supply-demand functions according to their costs. 


==> RelatedWork_v0.tex <==
\subsection{Related works (draft-version)}
%\textcolor{red}{Cong: this is citing form \cite{b1}\cite{b2} of this document. You can find the detail of "b1" by the end of the document "sn-article.tex". Eg: 	\bibitem{b1} Sepulveda, N.A., Jenkins, J.D., Edington, A. et al. The design space for long-duration energy storage in decarbonized power systems. Nat Energy 6, 506-516 (2021).}

Batteries' intrinsic costs may consist of multiple components: fixed costs, degradation costs, etc. But in the context of real-time or hourly operation, the dominant component is their opportunity costs: Charging power costs money, but it earns opportunities to sell back in the future, and vice versa. 


Many studies try to capture such opportunity costs of batteries through their bids, which in general falls into three  categories (shown by Fig.\ref{fig:bidcompare}). Type I is the quantity bid, which is the optimal self-scheduling of batteries as nondispatchable resources. Type II is the price-quantity bid, which uses bid-in prices to reveal both willingness to charge and discharge. Both Type I and Type II are grounded in the fact that many electricity markets permit batteries to submit quantity bids and price-quantity bids \cite{CAISO_StorageBid:21, ERCOT_storage:24}. Type III is the SOC-dependent bid from the recent proposal in California \cite{CAISO_SOCdependent:22}, which allows batteries submit different bid-in prices at different SOC levels. 

 
\begin{figure}[h]
	\centering
	\includegraphics[width=5.0in]{pic/bidcompare.png}
	\caption{Three types of storage bids: price forecast, computation, effectiveness, implementation.}
	\label{fig:bidcompare}
\end{figure}


Extensive Type I research captures battery opportunity cost through quantity bids \cite{shi18TACrainflow, HarshaDahleh15TPS, davies2019combined, ransan2021applying, beuse2021comparing, qin2023role}. They consider uncertainties from volatile energy market prices, maximize storage arbitrage opportunity profits in the objective function, and compute the optimal dispatch or control scheme for batteries. Thus, batteries bid its optimal scheduling plan as quantity bids directly into the electricity market as nondispatchable resources. 

Type II research usually captures battery opportunity cost through dynamic program \cite{JiangPowell15Storage, Lamadrid24JRE} and parametric program \cite{Alshehri&etal:20TPS, attarha23TEMPR}. They adopt the same stochastic program as Type I, but output the optimal scheduling plan as a function of electricity market price, which is the supply function and demand function. That way, batteries submit these functions representing their price-quantity bids to the electricity market. 


Recent Type III research runs in parallel with the industry's interest \cite{CAISO_DEB:20} to capture battery opportunity cost through SoC-dependent bids, \ie price vs. SOC \cite{ZhengXu22socAribitrage, Zhou&etal:24ACM}. However, SOC-dependent bids result in a computationally expensive non-convex market clearing problem replying on mixed integer programs (MIP) \cite{ZhengXu22energy}. Latest research in \cite{ChenTong22arXivSoC, Cong&Tong:22Allerton} convexifies the market clearing considering only the bid-in price's dependency over SOC. The computation burden and under-explored strategic behavior impedance the adoption of SOC-dependent bids in the electricity market. 
%Its unclear if the electricity market can effectively clear general SOC-dependent bids. %imposes extra limitations to the bidding format, restricting the effectiveness in revealing batteries willingness.
%The nonconvexity of the market clearing problem brought by the SOC-dependent bid also presents pricing challenges, resulting in out-of-merit dispatch and the need for out-of-the-market settlements in CAISO's real-time market. 

To summarize the pros and cons of different batteries' bids, quantity bids have the least computation complexity but strongly reply on accurate price forecasts. SOC-dependent bids don't reply on price forecast, but have the highest computation burden, limiting its application in industry. SOC dependent bids are the most effective when revealing batteries' charging and discharging willingness in multiple dimensions like the charging/discharging power and SOC levels. As is shown by Fig.\ref{fig:bidcompare}, price-quantity bids strike a balance in the spectrum for computation complexity and effectiveness in revealing batteries' willingness. Price-quantity bids also don't rely on price forecast. Therefore, we focus mainly on price-quantity bids in this paper.

%In Type IV, some new battery bidding formats like in \cite{bansal22EPSRrainflowmarket} is cleared by a convex energy market. However, this format limits the bid-in price to storage cycle depths, restricting the storage's ability to express its willingness to buy and sell energy across different SoC levels.





% \textcolor{red}{Cong: below is the references for this section}

% \bibitem{b1} K. Alshehri, M. Ndrio, S. Bose and T. Başar, "Quantifying Market Efficiency Impacts of Aggregated Distributed Energy Resources," in IEEE Transactions on Power Systems, vol. 35, no. 5, pp. 4067-4077, Sept. 2020, doi: 10.1109/TPWRS.2020.2979997. 


% \bibitem{b2} A. Attarha, M. Mahmoodi, S. M. N. R. A., P. Scott, J. Iria and S. Thiébaux, "Adjustable Price-Sensitive DER Bidding Within Network Envelopes," in IEEE Transactions on Energy Markets, Policy and Regulation, vol. 1, no. 4, pp. 248-258, Dec. 2023, doi: 10.1109/TEMPR.2023.3303911.

==> RelatedWork_v0_1.tex <==
 

Batteries' intrinsic costs may consist of multiple components: fixed costs \cite{peng2023heterogeneous,comello2019emergence}, degradation costs \cite{he2018intertemporal,levin2023energy},  etc. But in the context of real-time or hourly operation, the dominant component is their opportunity costs: Charging power costs money, but it earns opportunities to sell back in the future, and vice versa. \textcolor{red}{Many studies try to capture such opportunity costs of batteries through their bids, which in general fall into three categories (Fig.\ref{fig:bidcompare}). }

Type I is optimal self-scheduling

Type I is the quantity bid, the optimal self-scheduling of batteries as nondispatchable resources. Type II is \text{red}{the price-quantity bid}, also called the demand-supply function, \footnote{\text{red}{demand-supply curve}} which uses bid-in prices to reveal a willingness to charge and discharge. Both Type I and Type II are grounded in the fact that many electricity markets permit batteries to submit quantity bids and price-quantity bids \cite{CAISO_StorageBid:21, ERCOT_storage:24}. Type III is the SOC-dependent bid from the recent proposal in California \cite{CAISO_SOCdependent:22}, exploring batteries' different bid-in prices at different SOC levels. 

 
\begin{figure}[h]
	\centering
	\includegraphics[width=5.0in]{pic/bidcompare_v0.png}
	\caption{Related work for three types of storage bids. (From left to right listed sequentially Type I -Quantity bid, Type II - price-quantity bid/demand-supply function, and Type III - SoC-dependent bid. The computation burden and bidding effectiveness increase from Type I to Type III. ) }
	\label{fig:bidcompare}
\end{figure}


%Extensive Type I research captures battery opportunity cost through quantity bids \cite{shi18TACrainflow, HarshaDahleh15TPS, davies2019combined, ransan2021applying, beuse2021comparing, qin2023role}. They consider uncertainties from volatile energy market prices, maximize storage arbitrage opportunity profits in the objective function, and compute the optimal dispatch or control scheme for batteries. Thus, batteries bid its optimal scheduling plan as quantity bids directly into the electricity market as non-dispatchable resources. 

%Type II research usually captures battery opportunity cost through dynamic program \cite{JiangPowell15Storage, Lamadrid24JRE} and parametric program \cite{Alshehri&etal:20TPS, attarha23TEMPR}. They adopt the same stochastic program as Type I but output the optimal scheduling plan as a function of electricity market price, which is the supply function and demand function. That way, batteries submit these functions representing their price-quantity bids to the electricity market. 


%Recent Type III research runs in parallel with the industry's interest \cite{CAISO_DEB:20} to capture battery opportunity cost through SOC-dependent bids, i.e. price vs. SOC \cite{ZhengXu22socAribitrage, ChenTong22arXivSoC}. However, the computation burden and under-explored strategic behavior impedance the adoption of SOC-dependent bids in the electricity market.
%However, SOC-dependent bids result in a computationally expensive non-convex market clearing problem replying on mixed integer programs (MIP) \cite{ZhengXu22energy}. The latest research in \cite{ChenTong22arXivSoC} convexifies the market clearing considering only the bid-in price's dependency over SOC. 
% It's unclear if the electricity market can effectively clear general SOC-dependent bids. %imposes extra limitations on the bidding format, restricting the effectiveness of revealing batteries' willingness.
%The nonconvexity of the market clearing problem brought by the SOC-dependent bid also presents pricing challenges, resulting in out-of-merit dispatch and the need for out-of-the-market settlements in CAISO's real-time market. 

\textcolor{red}{Type I cannot reveal willingness to buy/sell under different price. Type II and III are parallel, internalize SOC, externalize SOC}


Here is a summary of the pros and cons of different batteries' bids. Type I quantity bids have the least computation complexity but strongly rely on accurate price forecasts \cite{HarshaDahleh15TPS, davies2019combined, ransan2021applying, beuse2021comparing, qin2023role}. Typical ways generally optimize storage arbitrage opportunity profits with a given price forecast to compute the optimal battery self-schedule. Type III SOC-dependent bids don't rely on the price forecast, and are the most effective when revealing batteries' charging and discharging willingness in multiple dimensions like the charging/discharging power and SOC levels. However, the highest computation burden and under-explored strategic behavior limit its application in practice \cite{CAISO_DEB:20, ZhengXu22socAribitrage, ChenTong22arXivSoC}. Type II price-quantity bids strike a balance in the spectrum for computation complexity and effectiveness in revealing batteries' willingness. Existing research usually captures battery opportunity cost through dynamic program \cite{JiangPowell15Storage, Lamadrid24JRE} and parametric program \cite{Alshehri&etal:20TPS, attarha23TEMPR}. \textcolor{red}{Price-quantity bids also don't rely on price forecasts.} Therefore, we focus mainly on price-quantity bids in this paper.

 

%In Type IV, some new battery bidding formats like in \cite{bansal22EPSRrainflowmarket} are cleared by a convex energy market. However, this format limits the bid-in price to storage cycle depths, restricting the storage's ability to express its willingness to buy and sell energy across different SoC levels.





% \textcolor{red}{Cong: below are the references for this section}

% \bibitem{b1} K. Alshehri, M. Ndrio, S. Bose and T. Başar, "Quantifying Market Efficiency Impacts of Aggregated Distributed Energy Resources," in IEEE Transactions on Power Systems, vol. 35, no. 5, pp. 4067-4077, Sept. 2020, doi: 10.1109/TPWRS.2020.2979997. 


% \bibitem{b2} A. Attarha, M. Mahmoodi, S. M. N. R. A., P. Scott, J. Iria and S. Thiébaux, "Adjustable Price-Sensitive DER Bidding Within Network Envelopes," in IEEE Transactions on Energy Markets, Policy and Regulation, vol. 1, no. 4, pp. 248-258, Dec. 2023, doi: 10.1109/TEMPR.2023.3303911.

==> method_v0.tex <==
\section{Methods}

We provide the base case and the proof of its demand-supply function in this method section. The generalized model to cases are also provided considering different battery efficiencies, energy dissipation, and ending SOC limit. Detailed proofs about the generalized demand-supply functions are provided in the supplemental material.

\subsection{Model used to generate the demand-supply function}
\subsubsection{Battery opportunity cost minimization}
To generate the demand-supply function of a battery, the following multi-period look-ahead optimization model is adopted as our basic model:
\begin{equation}\label{eq:M1_1}
	M_1: \min_{\{P,E\}} \,\, J =\sum_{t=1}^{T}{-c_t P_t \Delta t}
\end{equation}	
subject to the following constraints for $\forall t$: \begin{equation}\label{eq:M1_2}
	(\underline{\alpha}_t, \ \overline{\alpha}_t):\ -\overline{P} \leq P_t \leq \overline{P} 
\end{equation}			
%\begin{equation}\label{eq:M1_3}
%	(\underline{\alpha}^c_t, \ \overline{\alpha}^c_t):\ 0 \leq P^c_t \leq \overline{P^c}
%\end{equation}			
%\begin{equation}\label{eq:s}
%	P^d_tP^c_t=0 
%\end{equation}
\begin{equation}\label{eq:M1_3}
	(\sigma_t):E_{t+1} = E_1 - \sum_{\tau=1}^{t} P_\tau  \Delta t
\end{equation}	
\begin{equation}\label{eq:M1_4}
	(\underline{\beta}_t, \ \overline{\beta}_t):\ \underline{E} \leq E_{t} \leq \overline{E}
\end{equation}			
where $c_t$ is the electricity price at time $t$; $P_t$ is the net power output of the battery, for which positive means discharging and negative means charging. $E_t$ is the stored energy at time $t$ before the discharging and charging process at time $t$; $T$ is the number of time intervals in one day and $\Delta t$ is one time interval (can be calculated by $24/T$); $\overline{P}$ is the maximum discharging and charging power; $\overline{E}$ and $\overline{E}$ are the upper and lower limits of the stored energy; $E_1$ is the initial stored energy; $\underline{\alpha}^d_t$, $ \overline{\alpha}^d_t$, $\underline{\alpha}_t$  and  $\overline{\alpha}_t$  are the multipliers of the corresponding constraints. 

\par The objective in (\ref{eq:M1_1}) is the total cost of storage systems in one day. Constraints (\ref{eq:M1_2})  limit the upper and lower bounds of power;  constraint (\ref{eq:M1_3}) demonstrates the relationship between the stored energy at time $t$ and $t+1$ considering the charging and discharging process at time $t$; constraint (\ref{eq:M1_4}) limits the upper and lower bounds of the stored energy.


\subsubsection{Demand-supply function and Proof of Theorem \ref{BaseCaseTHM}}
The model in \eqref{eq:M1_1} is standard and widely adopted in the literature (cite). Given a set of battery parameters, future price forecast $c_2, ...c_T$, and an initial SOC $E_1$, we solve the optimal charging and discharging power with different prices for the current interval $c_1$ and formulate $P_1$ as a function of $c_1$. Such a function $P_1=f(c_1)$ is exactly the demand-supply function we study in this paper.

In Fig.~\ref{fig:5seg}, we provide the five segments example for the demand-supply function of battery, supported  by Theorem \ref{BaseCaseTHM}. Here we first provide the Lemma~\ref{BaseCaseN1less} and then finish the proof of Theorem \ref{BaseCaseTHM}.

\textcolor{red}{Could you finish the proof below with the simplified base case model (1)-(4)?}

Denote $T^B+1$ as the first time when $E_t$ is made to be bound by the inequality equation \eqref{eq:M1_4}, $n_c$ as the number of moments when $P_t=-\overline{P}, t \leq T^B$, $n_d$ as the number of moments when $P_t=\overline{P}, t \leq T^B$, $j$ as the moment when $-\overline{P} \leq P_t \leq \overline{P}$.
\newtheorem{lemma}{Lemma}
\begin{lemma}\label{BaseCaseN1less}
	\textit{There exists an optimal solution of $M1$ satisfying $T^B-n_c-n_d\leq1$.} 
\end{lemma}
\begin{proof}[Proof of Lemma~{\upshape\ref{BaseCaseN1less}}]
	First, the model $M_1$ can be divided into two models: the model when $t<T^B+1$ and the model when $t\geq T^B+1$. The model when $t<T^B+1$ denoted as $M_2$ can be written as follows:

\begin{equation}\label{eq:M2_1}
	M_2: \min_{\{P,E\}} \,\, J =\sum_{t=1}^{T^B}{-c_t P_t \Delta t}
\end{equation}	
subject to the following constraints: \begin{equation}\label{eq:M2_2}
	(\underline{\alpha}_t, \ \overline{\alpha}_t):\ -\overline{P} \leq P_t \leq \overline{P}, \forall t\leq T^B
\end{equation}			
\begin{equation}\label{eq:M2_3}
	(\mu):E_{T^B+1} = E_1 - \sum_{\tau=1}^{t} P_\tau  \Delta t
\end{equation}	

Let $L$ be a Lagrangian function and according to the KKT condition we have

\begin{equation}\label{eq:M2_L}
    \frac{dL}{dP_t} = -c_t \Delta t - \underline{\alpha_t} + \overline{\alpha_t} + \mu \Delta t = 0
\end{equation}	
 
\par Then, we prove the lemma by contradiction. We assume that there exists an optimal solution satisfying $T^B-n_c-n_d=n>1$, where $n$ is the number of moments for which $-\overline{P} < P_t < \overline{P}$ and the number of moments and the set of these moments is defined as $T^n$. When $-\overline{P} < P_t < \overline{P}$, $\underline{\alpha_t} = \overline{\alpha_t} =0$ holds. By substituting $\underline{\alpha_t} = \overline{\alpha_t} =0$ into \eqref{eq:M2_L}, $c_t=\mu$ holds. This means the electricity prices at the $n$ time points are equal when the hypothesis holds. Let $c^n$ denote the electricity price at these time points.
\par Then, the objective function \eqref{eq:M2_1} can be expressed as:

\begin{equation}\label{eq:M2_1_1}
    J = -c^n \sum_{t \in T^n} P_t \Delta t - \sum_{t \notin T^n} c_t P_t \Delta t.
\end{equation}	
And constraint \eqref{eq:M2_3} can be expressed as:
\begin{equation}\label{eq:M2_3_1}
	(\mu):E_{T^B+1} = E_1 - \sum_{t \in T^n} P_t \Delta t-\sum_{t \notin T^n} P_t \Delta t.
\end{equation}	
At this stage, the optimization of $M^B$ hinges on the aggregate term $\sum_{t \in T^n} P_t \Delta t$. For the optimal solution of $\sum_{t \in T^n} P_t \Delta t$, an infinite number of combinations of $P_t$ values exist for $t \in T^n$. Crucially, it is always feasible to identify a set of values ensuring that at most one time point is neither fully charged nor fully discharged. Therefore, it is always possible to find an optimal solution that $T^B-n_c-n_d\leq1$ holds.
\end{proof} 


\begin{lemma}\label{BaseCaselemma2}
	\textit{Given the parameters $\{E_1, c, T, \underline{E}, \overline{E}, \overline{P}\}$, if for $M_1$ there exists $T^B$ such that $E_{T^B+1} = \underline{E}$, then as $c_1$ increases, there will be no $T^B$ such that $E_{T^B+1} = \overline{E}$ holds.
} 
\end{lemma}
\begin{proof}[Proof of Lemma~{\upshape\ref{BaseCaselemma2}}]
$M_3$ can be regarded as the problem of finding the optimal solution for times $t = 2$ to $T$, given that the optimal solution at $t = 1$ is known. When $\{E_1, c, T, \underline{E}, \overline{E}, \overline{P}\}$ remain unchanged, the optimal solution of $M_3$ is optimal in $M_1$. Based on the non-decreasing characteristic of the energy storage price response function, as $c_1$ increases, $P_1$ either remains unchanged or increases. Therefore, in $M_3$, $E_2$ decreases, meaning that the initial energy storage level decreases. If there originally existed $T^B$ such that $E_{T^B+1} = \underline{E}$, when other parameters remain unchanged and $E_2$ decreases, there will not exist a $T^B$ such that $E_{T^B+1} = \overline{E}$.
\end{proof}


\begin{proof}[Proof of Theorem~{\upshape\ref{BaseCaseTHM}}]

    \par First, by utilizing the properties of multi-parametric linear programming, a proof of the staircase property is conducted. The dual problem of $M_1$ is as follows: 
    \begin{equation}
        M_{1,\text{(dual)}}:  \min_{u} \, W = b'u 
    \end{equation}   
    subject to
    \begin{equation}
        (P): \, G'u \leq c 
    \end{equation}
    According to the properties of the multi-parametric linear programming problem (MPLP) (Theorem 6.5 in \cite{borrelli2017predictive}), for $M_{1,\text{(dual)}}$, the function $W^*(c)$ is a piecewise affine convex function (with the electricity price $c$ as a parameter). Therefore, the function $P(c) = \frac{\partial W^*(c)}{\partial c}$ is a stepwise monotonic non-decreasing function.

	\par Second, for the optimal solution of the model $M_1$, there are at most 5 segments: 
	\par For Case1: $T^B-n_c-n_d=0$ or $T^B-n_c-n_d=1, j=1$ holds. Therefore, $P_{1,\text{(case1)}}\in \{-\overline{P},\overline{P}\}$ corresponds to two kinds of segments, which are the fully-charge and the fully-discharge segments, denoted by $P_{s1}$ and $P_{s5}$ respectively; 
    \par For Case2: $T^B-n_c-n_d=1, j\neq1$ holds. According to Lemma~\ref{BaseCaseN1less} and (\ref{eq:M2_3}),
	\begin{equation}\label{eq:Theorem1_1}
		P_{1,\text{(case2)}} = \frac{E_1 - E_{T^B+1}}{\Delta t} - (n_d - n_c)\overline{P}
	\end{equation}
	holds. Four segments can be derived by \eqref{eq:Theorem1_1}: 
    \begin{itemize}
         \item  When $P_{1,\text{(case2)}}\leq 0$, this is a charging segment: 
         \begin{itemize}
           \item $P_{s2}$: when $E_{T^B+1}=\overline{E}$, this is the Charge-for-charge segment;
          \item $P_{s3}^C$: when $E_{T^B+1}=\underline{E}$, this is the Charge-for-discharge segment.
         \end{itemize}
         \item  When $P_{1,\text{(case2)}}\geq 0$, this is a discharging segment: 
        \begin{itemize}
          \item $P_{s3}^D$: when $E_{T^B+1}=\overline{E}$, this is the Discharge-for-charge segment;
          \item $P_{s4}$: when $E_{T^B+1}=\underline{E}$, this is the Discharge-for-discharge segment.
         \end{itemize}
    \end{itemize}
    \par Then, according to Lemma~\ref{BaseCaselemma2}, $P_{s3}^C$ and $P_{s4}^D$ can not appears simultaneously. Therefore, the total number of segments is at most 5.  
\end{proof}	 


\subsection{Model Generalization and demand-supply function}

\subsubsection{Different charging and discharging efficiencies}
Denote  $\overline{P^d}$ and $\overline{P^c}$ as the maximum discharging and charging power, and $\eta^d$ and $\eta^c$ as discharging and charging efficiencies. Constraints of base cases changes to ...   $\forall t$: 
\begin{equation}\label{eq:2d}
	(\underline{\alpha}^d_t, \ \overline{\alpha}^d_t):\ 0 \leq P^d_t \leq \overline{P^d} 
\end{equation}			
\begin{equation}\label{eq:2c}
	(\underline{\alpha}^c_t, \ \overline{\alpha}^c_t):\ 0 \leq P^c_t \leq \overline{P^c}
\end{equation}			
\begin{equation}\label{eq:s}
	P^d_tP^c_t=0 
\end{equation}
\begin{equation}\label{eq:t}
	(\sigma_t):E_{t+1} = E_1 - \sum_{\tau=1}^{t}(\frac{P^d_\tau}{\eta^d} - P^c_\tau \eta^c)\Delta t
\end{equation}	

\par  Constraints (\ref{eq:2d}) and (\ref{eq:2c}) limit the upper and lower bounds of power; constraint (\ref{eq:s}) limits that the storage system can not discharge and charge simultaneously at time $t$; constraint (\ref{eq:t}) demonstrates the relationship between the stored energy at time $t$ and $t+1$ considering the charging and discharging process at time $t$; constraint (\ref{eq:4}) limits the upper and lower bounds of the stored energy.


\subsubsection{energy dissipation}
When energy dissipation is considered, constraint (\ref{eq:t}) changes to ...

...

where

When the ending SOC is limited, the following equality constraint will be adde
\begin{equation}\label{eq:5a}
	(\mu):E_{T+1}=E_1 ,
\end{equation}		
which means the stored energy after the discharging and charging process should return to the initial value $E_1$.


\subsubsection{Ending SOC limit}

The standard model tends to discharge energy to its lower bound since only the total profit is considered in the objective function. To address this issue, we can specify that the energy at time $T+1$ should be no lower than a given threshold, e.g., let $S_{T+1}\geq S_0$. This may introduce two additional stairs corresponding to two new remainder energy levels. Please see Fig.\ref{fig:figy} as examples.


\begin{figure}[H]
	\centering
	\includegraphics[width=2.0in]{pic/endingSOClimit.png}
	\caption{Impact of \textbf{the ending SOC limit} on the demand-supply functions of the energy storage system(the capacity is 2MWh, the maximum charging/discharging power is 0.6MW, the upper and lower bounds of SOC are 1 and 0.1, the initial SOC is 0.5, the total number of time periods is 24 with one time period being 1 hour) under extreme prices shown in Fig.\ref{fig:figx}(c). In (a) there are three kinds of stairs, which is the same with Fig.\ref{fig:figx}(f). In (b) there are seven kinds of stairs, and compared with Fig.\ref{fig:figx}(i) it can be observed that new discharging and charging stairs appear. In (c) there are six kinds of stairs, which is the same with Fig.\ref{fig:figx}(l).}
	\label{fig:figy}
\end{figure}
 


%\subsubsection{Different charging and discharging maximum capacity limits}




\section{Supplemental Materials}

\textcolor{red}{May be we will show the most complicated complete model here first and explain the generalization to all these cases one by one.}

\subsection{Relaxation of $M1$}
We define the model with (\ref{eq:s}) relaxed, i.e., removed from $M1$, as $M2$. The sufficient condition for the exact relaxation is proposed and proved in this subsection.
\begin{theorem}\label{thm1}
	\textit{Assume $c_t>0$ holds for $\forall t$, the optimal solutions of decision variables in $M2$ is also optimal for $M1$.}
\end{theorem}

\par Proof of Theorem \ref{thm1} can be found in Appendix \ref{secA1}. The exactness of the $M2$ can be interpreted intuitively: with $c_t>0$ satisfied, charging and discharging simultaneously will waste energy. It is uneconomic for a storage system since the wasted energy should be charged back with $c_t$ which increases the cost. Therefore, the optimal solution in $M2$ still implicitly satisfies the constraint (\ref{eq:s}). 


\begin{theorem}\label{thm2}
	\textit{Assume there exists a feasible solution for M2. The function of the demand-supply function $P_1=f(c_1)$ is staircase and monotonically non-decreasing.}
\end{theorem}
Proof of Theorem \ref{thm2} can be found in Appendix \ref{secA2}.



\par The time interval at which $E_t$ is bound by an equality equation for the first time is defined as $T^B+1$. The equality equation can be $E_{T^B+1}=\underline{E}$, $E_{T^B+1}=\overline{E}$ and $E_{T^B+1}=E_1$. $n_c$ is defined as the number of time intervals when $P_t=\overline{P^c}, t\leq T^B$; $n_d$ is defined as the number of time intervals when $P_t=\overline{P^d}, t\leq T^B$; $n_0$ is defined as the number of time intervals when $P_t=0, t\leq T^B$.
\newtheorem{lemma}{Lemma}
\begin{lemma}\label{lem1}
	\textit{There exists an optimal solution of $M2$ which satisfies $T^B-n_c-n_d-n_0\leq1$.} 
\end{lemma}
Proof of Lemma \ref{lem1} can be found in Appendix \ref{secA3}.


\begin{theorem}\label{thm3}
\textit{When parameters of $\{E_1$, $c$, $\eta^d$, $\eta^c$, $T$, $\underline{E}$, $\overline{E}$, $\overline{P^d}$, $\overline{P^c}\}$ are given, the number of kinds of segments in the demand-supply functions is no more than 9.}
\end{theorem}
Proof of Theorem \ref{thm3} can be found in Appendix \ref{secA4}.

\subsection{Parameter Sensitivities}

Formally presented by the following theorem:

\begin{theorem}
    Consider a battery whose decision model is presented in (M1). For any point ($c_1$,$P_1$) on its original supply-demand curve, there exists an $\alpha$ such that the point ($c_1+\alpha$,$P_1$) is on its new curve when its future price forecast changes to $c_2'...c_T'$ and all other quantities do not change, and there exists an $\beta$ such that the point ($c_1$,$P_1+\beta$) is on its new curve when its initial SOC $E_1$ changes to $E_1'$ and all other quantities do not change.
\end{theorem}


==> method_v0_1.tex <==
\section{Methods}

We first provide the base case and the proof of its demand-supply function in this method section. Then generalizations are provided considering different battery efficiencies, energy dissipation, and ending SOC limit. Detailed proofs about the generalized demand-supply functions are provided in the supplemental material.

\subsection{Model used to generate the demand-supply function}
\subsubsection{Battery opportunity cost minimization}
To generate the demand-supply function of a battery, the following multi-period look-ahead optimization model is adopted as our basic model:
\begin{equation}\label{eq:M1_1}
	M_1: \min_{\{P,E\}} \,\, J =\sum_{t=1}^{T}{-c_t P_t \Delta t}
\end{equation}	
subject to the following constraints for $\forall t$: \begin{equation}\label{eq:M1_2}
	(\underline{\alpha}_t, \ \overline{\alpha}_t):\ -\overline{P} \leq P_t \leq \overline{P} 
\end{equation}			
%\begin{equation}\label{eq:M1_3}
%	(\underline{\alpha}^c_t, \ \overline{\alpha}^c_t):\ 0 \leq P^c_t \leq \overline{P^c}
%\end{equation}			
%\begin{equation}\label{eq:s}
%	P^d_tP^c_t=0 
%\end{equation}
\begin{equation}\label{eq:M1_3}
	(\sigma_t):E_{t+1} = E_1 - \sum_{\tau=1}^{t} P_\tau  \Delta t
\end{equation}	
\begin{equation}\label{eq:M1_4}
	(\underline{\beta}_t, \ \overline{\beta}_t):\ \underline{E} \leq E_{t} \leq \overline{E}
\end{equation}			
where $c_t$ is the electricity price at time $t$; $P_t$ is the net power output of the battery, for which positive means discharging and negative means charging. $E_t$ is the stored energy at time $t$ before the discharging and charging process at time $t$; $T$ is the number of time intervals in one day and $\Delta t$ is one time interval (can be calculated by $24/T$); $\overline{P}$ is the maximum discharging and charging power; $\overline{E}$ and $\underline{E}$ are the upper and lower limits of the stored energy; $E_1$ is the initial stored energy;  $\underline{\alpha}_t$  and  $\overline{\alpha}_t$  are the multipliers of the corresponding constraints. 

\par The objective in (\ref{eq:M1_1}) is the total cost of storage systems in one day. Constraints (\ref{eq:M1_2})  limit the upper and lower bounds of power;  constraint (\ref{eq:M1_3}) demonstrates the relationship between the stored energy at time $t+1$ considering the charging and discharging process before time $t+1$; constraint (\ref{eq:M1_4}) limits the upper and lower bounds of the stored energy.


\subsubsection{Demand-supply function and Proof of Theorem \ref{BaseCaseTHM}}
The model in \eqref{eq:M1_1} is standard and widely adopted in the literature (cite). Given a set of battery parameters, future price forecast $c_2, ...c_T$, and an initial SOC $E_1$, we solve the optimal charging and discharging power with different prices for the current interval $c_1$ and formulate $P_1$ as a function of $c_1$. Such a function $P_1=f(c_1)$ is exactly the demand-supply function we study in this paper.

In Fig.~\ref{fig:5seg}, we provide the five segments example for the demand-supply function of battery, supported by Theorem \ref{BaseCaseTHM}. Here we first provide the Lemma~\ref{BaseCaseN1less} and  Lemma~\ref{BaseCaselemma2}. Then we finish the proof of Theorem \ref{BaseCaseTHM}.

%\textcolor{red}{Could you finish the proof below with the simplified base case model (1)-(4)?}

Denote $T^B+1$ as the first time we have the binding inequality constraint \eqref{eq:M1_4}, $n_c$ as the number of intervals when $P_t=-\overline{P}, \forall t \leq T^B$,  and $n_d$ as the number of intervals when $P_t=\overline{P}, \forall t \leq T^B$. Denote $j$ as the time index  when $-\overline{P} < P_t < \overline{P}, t\le T^B$. An example of these terms are shown in Fig.\ref{fig:denotation_of_terms}.
\begin{figure}[h]
	\centering
	\includegraphics[width=5.0in]{pic/denotation of terms.png}
	\caption{An Example of $T^B+1$, $n_c$, $n_d$, and $j$.}
	\label{fig:denotation_of_terms}
\end{figure}

\newtheorem{lemma}{Lemma}
\begin{lemma}\label{BaseCaseN1less}
	\textit{There exists an optimal solution of $M_1$ satisfying $T^B-n_c-n_d\leq1$.} 
\end{lemma}
\begin{proof}[Proof of Lemma~{\upshape\ref{BaseCaseN1less}}]
	
We prove this lemma by contradiction. Suppose there exist more than one time interval such that $-\overline{P} < P_t < \overline{P}$, i.e. $\Omega:=\{t\le T^B|-\overline{P} < P_t < \overline{P}\}$, $N:=|\Omega|, N>1$.
  
From the KKT condition of $M_1$, we have:
%$\rho_t=\sum_{t'=t}^{T^B} (\underline{\beta}-\overline{\beta})$.
\begin{align}
    &\frac{\partial L}{\partial P_t} = -c_t \Delta t - \underline{\alpha_t} + \overline{\alpha_t} + \sum_{\tau\geq t}{\sigma_{\tau} \Delta t} = 0, \ \forall t \in [1,T]. \label{eq:omegaKKT_P} \\
    &\frac{\partial L}{\partial E_t} = \sigma_{t-1} -\underline{\beta}_t + \overline{\beta}_t= 0, \ \forall t \in [2,T+1]. \label{eq:omegaKKT_E}
\end{align}
\par Since $T^B+1$ is the first time interval when the inequality constraint \eqref{eq:M1_4} is binding, $\underline{\beta_t}= \overline{\beta_t}=0, \forall t\le T^B$. Therefore, $\sigma_t =0, \forall t\le T^B$ holds. And when $t\in \Omega$, $\underline{\alpha}_t=\overline{\alpha}_t=0$ holds. 
Then, by substituting $\sigma_t =0, \underline{\alpha}_t=\overline{\alpha}_t=0, \forall t\in \Omega$ into \eqref{eq:omegaKKT_P}, we have
\begin{equation}\label{eq:omegaKKT_P_omega}
    \frac{\partial L}{\partial P_t} = -c_t \Delta t + \sigma_{T^B} \Delta t = 0, \ \forall t \in \Omega. \Rightarrow c_t=\sigma_{T^B}, \forall t\in \Omega.
\end{equation}
%Therefore, $c_t=\sigma_{T^B}, \forall t\in \Omega$. 
    %-c^n \sum_{t \in T^n} P_t \Delta t = \mu (\sum_{t \in T^n} P_t \Delta t)
% that satisfying the objective function and all constraints, i.e. $\sum_{t \in \Omega} \hat{P}_t \Delta t = \sum_{t \in \Omega} P_t \Delta t$.
\par Denote $N':=\lfloor{\frac{|\sum_{t \in \Omega} P_t|}{\overline{P}}}\rfloor$. We have $N' \overline{P}\leq |\sum_{t \in \Omega} P_t| < (N'+1)\overline{P}$. Then the following equations can be derived:
\begin{align}
    0 \leq  -N' \overline{P}+ \sum_{t \in \Omega} P_t < \overline{P}, if \sum_{t \in \Omega} P_t & \geq 0; \label{eq:lem1N'ge0} \\
    -\overline{P} < N' \overline{P}+ \sum_{t \in \Omega} P_t\leq 0, if  \sum_{t \in \Omega} P_t & \leq 0. \label{eq:lem1N'le0}
\end{align}
We define $\{\hat{P}_t\}_{t \in \Omega}$ by the following four cases:
\begin{itemize}
    \item Case1: There exists an integer $n$ that satisfies $N=N'+2n$:
    \begin{itemize}
        \item Case1.A: $\sum_{t \in \Omega} P_t\geq 0$: for $t=j$, $\hat{P}_j= -(N'+1) \overline{P}+\sum_{t \in \Omega} P_t$ and let $j$ be the smallest time index in $\Omega$. Then by adding $-\overline{P}$ to \eqref{eq:lem1N'ge0} simultaneously, $-\overline{P} \leq -(N'+1) \overline{P}+ \sum_{t \in \Omega} P_t< 0$ holds. Then we have $\hat{P}_j \in [-\overline{P}, 0)$. For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, for the smallest $2n-2$ time indexes in $\Omega$ except $j$, $\overline{P}$ and $-\overline{P}$ are set by turns according the order of the time index; for the largest $N'+1$ time indexes, $\overline{P}$ are set. %\textcolor{red}{For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, we randomly assign $N'+n$ of them to be $\overline{P}$ and $n-1$ of them to be $-\overline{P}$. According to Cong: I notice that we cannot randomly assign, we need to make it satisfy the SoC limit constraints. Could you provide the assigning details that satisfy the constraint?}% \textcolor{red}{Cong's revision: did you show that ?} %\textcolor{red}{; Cong: you need to specify which $\hat{P}_t$ is $\overline{P}$ and which one goes to $-\overline{P}$. Define $\{\hat{P}_t\}_{t \in \Omega}$ precisely. Similar modifications are needed for all other cases.}
        \item Case1.B: $\sum_{t \in \Omega} P_t\leq 0$: $\hat{P}_j= (N'+1) \overline{P}+\sum_{t \in \Omega} P_t$. Then by adding $\overline{P}$ to \eqref{eq:lem1N'le0} simultaneously, $0 < -(N'+1) \overline{P}+ \sum_{t \in \Omega} P_t \leq \overline{P}$ holds. Then we have $\hat{P}_j \in (0, \overline{P}]$. For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, for the smallest $2n-2$ time indexes in $\Omega$ except $j$, $-\overline{P}$ and $\overline{P}$ are set by turns according the order of the time index; for the largest $N'+1$ time indexes, $-\overline{P}$ are set. %For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, we randomly assign $n-1$ of them to be $\overline{P}$ and $N'+n$ of them to be $-\overline{P}$.
    \end{itemize}
    \item Case2: There exists an integer $n$ that satisfies $N=N'+2n+1$:
    \begin{itemize}
        \item Case2.A: $\sum_{t \in \Omega} P_t\geq 0$: $\hat{P}_j= -N' \overline{P}+\sum_{t \in \Omega} P_t$. According to \eqref{eq:lem1N'ge0}, we have $\hat{P}_j \in [0,\overline{P})$. For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, for the smallest $2n$ time indexes in $\Omega$ except $j$, $-\overline{P}$ and $\overline{P}$ are set by turns according the order of the time index; for the largest $N'$ time indexes, $\overline{P}$ are set. %For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, we randomly assign $N'+n$ of them to be $\overline{P}$ and $n$ of them to be $-\overline{P}$.
        \item Case2.B: $\sum_{t \in \Omega} P_t\leq 0$: $\hat{P}_j= N' \overline{P}+\sum_{t \in \Omega} P_t$. According to \eqref{eq:lem1N'le0}, we have $\hat{P}_j \in (-\overline{P},0]$. For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, for the smallest $2n$ time indexes in $\Omega$ except $j$, $\overline{P}$ and $-\overline{P}$ are set by turns according the order of the time index; for the largest $N'$ time indexes, $\overline{P}$ are set. %For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, we randomly assign $n$ of them to be $\overline{P}$ and $N'+n$ of them to be $-\overline{P}$.
    \end{itemize}
\end{itemize}
 % $\hat{P}_t, t \in \Omega$
For $\{\hat{P}_t\}_{t \in \Omega}$, we can easily show that (i) $\hat{\Omega}:=\{t\le T^B|-\overline{P} < \hat{P}_t < \overline{P}\}$, $|\hat{\Omega}|\le 1$; (ii) $\hat{P}_t, t \in \Omega$ is an equal optimal solution to $P_t, t \in \Omega$, because they achieve the same  objective value and satisfy all constraints

% By analyzing all possible cases of $\hat{P}_t, t \in \Omega$, $\hat{\Omega}:=\{t\le T^B|-\overline{P} < \hat{P}_t < \overline{P}\}$, $|\hat{\Omega}|\le 1$. hat satisfying the objective function and all constraints, 

Therefore, it is always possible to find an optimal solution that $T^B-n_c-n_d\leq1$ holds.
\end{proof} 


\begin{lemma}\label{BaseCaselemma2}
	\textit{Given the parameters $\{E_1, c, T, \underline{E}, \overline{E}, \overline{P}\}$, if for $M_1$ there exists $T^B$ such that $E_{T^B+1} = \underline{E}$, then as $c_1$ increases, there will be no $T^B$ such that $E_{T^B+1} = \overline{E}$ holds.
} 
\end{lemma}
\begin{proof}[Proof of Lemma~{\upshape\ref{BaseCaselemma2}}]
$M_3$ can be regarded as the problem of finding the optimal solution for times $t = 2$ to $T$, given that the optimal solution at $t = 1$ is known. When $\{E_1, c, T, \underline{E}, \overline{E}, \overline{P}\}$ remain unchanged, the optimal solution of $M_3$ is optimal in $M_1$. Based on the non-decreasing characteristic of the energy storage supply-demand function, as $c_1$ increases, $P_1$ either remains unchanged or increases, resulting in the energy consumption at $t=1$ remaining unchanged or increasing. Therefore, $E_2$, i.e. the initial energy storage level in $M_3$, remains unchanged or decreases. Suppose there originally existed $T^B$ such that $E_{T^B+1} = \underline{E}$, when other parameters remain unchanged and $E_2$ remains unchanged, the energy in the battery will be fully discharged at $T^B+1$; when $E_2$ decreases, the energy in the battery will be fully discharged at $T^B+1$ or before $T^B+1$. In any of these cases, the battery will not be fully charged before it has been fully discharged. Therefore, there will not exist a $T^B$ such that $E_{T^B+1} = \overline{E}$.
\end{proof}


\begin{proof}[Proof of Theorem~{\upshape\ref{BaseCaseTHM}}]

    \par First, by utilizing the properties of multi-parametric linear programming, a proof of the staircase property is conducted. The dual problem of $M_1$ is as follows: 
    \begin{equation}
        M_{1,\text{(dual)}}:  \min_{u} \, W = b'u 
    \end{equation}   
    subject to
    \begin{equation}
        (P): \, G'u \leq c 
    \end{equation}
    According to the properties of the multi-parametric linear programming problem (MPLP) (Theorem 6.5 in \cite{borrelli2017predictive}), for $M_{1,\text{(dual)}}$, the function $W^*(c)$ is a piecewise affine convex function (with the electricity price $c$ as a parameter). Therefore, the function $P(c) = \frac{\partial W^*(c)}{\partial c}$ is a stepwise monotonic non-decreasing function.

	\par Second, for the optimal solution of the model $M_1$, there are at most 5 segments: 
% \textcolor{blue}{ \begin{equation}
%          P_1(c_1)=\begin{cases} -\overline{P},& \text{if}~ c_1\le c_1^a,\\
%          \frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P},& \text{if}~ c_1^a < c_1\le  c_1^b,\\
%          \frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}~\text{or}~ \frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P},& \text{if}~ c_1^b < c_1\le  c_1^c,\\
%          \frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P},& \text{if}~ c_1^c< c_1 \le c_1^d,\\
%          \overline{P},& \text{if}~ c_1\ge  c_1^d,\\
%      \end{cases}
%  \end{equation}
%  where $n_d$ and $n_c$ are functions of $c_1$.}
 
From Lemma~\ref{BaseCaseN1less},  $j \in \{\emptyset,1, 2, ..., T^B\}$.

	\par For Case1: $T^B-n_c-n_d=0$ or $T^B-n_c-n_d=1, j\neq 1$ holds. Therefore, $P_{1,\text{(case1)}}\in \{-\overline{P},\overline{P}\}$ corresponds to two kinds of segments, which are the fully-charge and the fully-discharge segments, denoted by $P_{s1}=-\overline{P}$ and $P_{s5}=\overline{P}$ respectively;


% \textcolor{blue}{Denote $c_1^d$ be the value such that $T^B-n_c-n_d=1, j=1$.}
    \par For Case2: $T^B-n_c-n_d=1, j=1$ holds. We know $P_1 \in (-\overline{P}, \overline{P})$, and according to Lemma~\ref{BaseCaseN1less}, we have $\{P_t\}_{t=2}^{T^B} \in \{-\overline{P}, \overline{P}\}$.  \begin{align}
    \begin{aligned}
        &E_{T^B+1} \overset{(a)}{=} E_1 - \sum_{\tau=1}^{t} P_\tau  \Delta t \overset{(b)}{=} E_1 - (n_d - n_c)\overline{P}+ P_{1,\text{(case2)}}, \\
         \overset{(c)}{\Rightarrow} &P_{1,\text{(case2)}} = \frac{E_1 - E_{T^B+1}}{\Delta t} - (n_d - n_c)\overline{P} \Delta t .
        \end{aligned}
    \end{align} 
    where (a) comes from  (\ref{eq:M1_3}); (b) comes from the definition of $n_d, n_c$, $P_1 \in (-\overline{P}, \overline{P})$, and $\{P_t\}_{t=2}^{T^B} \in \{-\overline{P}, \overline{P}\}$;   (c) can be derived by moving elements around the equation.
    
    According to Lemma~\ref{BaseCaseN1less} and (\ref{eq:M1_3}),
	\begin{equation}\label{eq:Theorem1_1}
		P_{1,\text{(case2)}} = \frac{E_1 - E_{T^B+1}}{\Delta t} - (n_d - n_c)\overline{P}
	\end{equation}
	holds. Four segments can be derived by \eqref{eq:Theorem1_1}: 
    \begin{itemize}
         \item  When $P_{1,\text{(case2)}}\leq 0$, this is a charging segment: 
         \begin{itemize}
           \item $P_{s2}=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P}$, this is the Charge-for-charge segment; %\textcolor{red}{Cong: if one equation is definition, then you need to write $P_{s2}:=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P}$.}
          \item $P_{s3}^C=\frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}$, this is the Charge-for-discharge segment.
         \end{itemize}
         \item  When $P_{1,\text{(case2)}}\geq 0$, this is a discharging segment: 
        \begin{itemize}
          \item $P_{s3}^D=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P}$, this is the Discharge-for-charge segment;
          \item $P_{s4}=\frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}$, this is the Discharge-for-discharge segment.
         \end{itemize}
    \end{itemize}
    \par Note that according to constraints \eqref{eq:M1_2}, we have:
    \begin{align}
        -\overline{P}&<P_{s2}\leq 0 \label{eq:the1_ncnd_ps2} \\
        -\overline{P}&<P_{s3}^C\leq 0 \label{eq:the1_ncnd_ps3C} \\
        0&\leq P_{s3}^D < \overline{P} \label{eq:the1_ncnd_ps3D} \\
        0&\leq P_{s4}< \overline{P} \label{eq:the1_ncnd_ps4} 
    \end{align}
    Then by substituting $P_{s2}=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P}$ into \eqref{eq:the1_ncnd_ps2}, we have \eqref{eq:the1_ncnd_ps2_re}; by substituting $P_{s3}^C=\frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}$ into \eqref{eq:the1_ncnd_ps3C}, we have \eqref{eq:the1_ncnd_ps3C_re}; by substituting $P_{s3}^D=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P}$ into \eqref{eq:the1_ncnd_ps3D}, we have \eqref{eq:the1_ncnd_ps3D_re}; by substituting $P_{s4}=\frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}$ into \eqref{eq:the1_ncnd_ps4}, we have \eqref{eq:the1_ncnd_ps4_re}.
    \begin{align}
        &\text{for} P_{s2}: \frac{E_1-\overline{E}}{\overline{P} \Delta t} \leq n_d-n_c <\frac{E_1-\overline{E}}{\overline{P}\Delta t} +1 \label{eq:the1_ncnd_ps2_re} \\
        &\text{for} P_{s3}^C: \frac{E_1-\underline{E}}{\overline{P} \Delta t} \leq n_d-n_c <\frac{E_1-\underline{E}}{\overline{P}\Delta t} +1 \label{eq:the1_ncnd_ps3C_re} \\
        &\text{for} P_{s3}^D: \frac{E_1-\overline{E}}{\overline{P} \Delta t} -1 < n_d-n_c \leq \frac{E_1-\overline{E}}{\overline{P}\Delta t} \label{eq:the1_ncnd_ps3D_re} \\
        &\text{for} P_{s4}: \frac{E_1-\underline{E}}{\overline{P} \Delta t} -1 < n_d-n_c \leq \frac{E_1-\underline{E}}{\overline{P}\Delta t} \label{eq:the1_ncnd_ps4_re} 
    \end{align}
    Here, if we denote $\frac{E_1-\overline{E}}{\overline{P} \Delta t}$ as $K$, we have $K \leq n_d-n_c<K+1$. Since $n_d-n_c$ is an integer, for \eqref{eq:the1_ncnd_ps2_re} only one value exists for $n_d-n_c$. Similarly, for \eqref{eq:the1_ncnd_ps3C_re}, \eqref{eq:the1_ncnd_ps3D_re} and \eqref{eq:the1_ncnd_ps4_re}, there exists only one $n_d-n_c$ for each of them. %\textcolor{red}{Cong: You only show $P_s2$-$P_s4$ are four constants. Did you show that $P_s2$-$P_s4$ are different values?} \textcolor{purple}{Chenge: Sometimes, values of $P_{s2}$ and $P_{s3}^C$ are equal, values of $P_{s4}$ and $P_{s3}^D$ are equal. For example when Emax=20MWh, Emin=0, Pmax=5MW, E1=12.5MWh. We have $P_{s2}=P_{s3}^C=-2.5$ and $P_{s4}=P_{s3}^D=2.5$. Therefore, the values of stairs may be equal. I've tried, but proving that $P_s2$-$P_s4$ are different values is difficult. Now we have different functions of them, do you think it is enough?}  
    Therefore,  $P_{s2}$, $P_{s3}^C$, $P_{s3}^D$, and $P_{s4}$ are four constants. %\textcolor{red}{It is noted that there exists at most one value of $n_d-n_c$ for each of \eqref{eq:the1_ncnd_ps2_re}-\eqref{eq:the1_ncnd_ps4_re}.  Cong: how can you see this? D you need to prove like for $P_{s4}$, the gap between upper and lower bounds has $ k-1 < \frac{E_1-\underline{E}}{\overline{P}\Delta t} - \frac{E_1-\underline{E}}{\overline{P} \Delta t} < k+1$?} 
%    In Fig.XX, we present the example with all four different constants, construct four . }    
    \par Until now we prove six constants $P_{s1}$, $P_{s2}$, $P_{s3}^C$, $P_{s3}^D$,  $P_{s4}$, and $P_{s5}$ constructing the segments in the stair functions $P_1(c_1)$. According to Lemma~\ref{BaseCaselemma2}, $P_{s3}^C$ and $P_{s4}^D$ can not appears simultaneously.  In Sec.\ref{sec_example_5}, we present an example with five segments exist. Therefore, the total number of segments is at most five. %And when no $n_d-n_c$ satisfies any of \eqref{eq:the1_ncnd_ps2_re}-\eqref{eq:the1_ncnd_ps4_re}, corresponding segments $P_{s2}$, $P_{s3}^C$, $P_{s3}^D$, and $P_{s4}$ will not exist. And if the initial SOC is not enough for fully charging or discharging for one time interval, the corresponding fully charge segment $P_{s1}$ or fully discharge segment $P_{s5}$ will not exist. Therefore, the total number of segments is at most 5.  
\end{proof}	 

\subsubsection{An example of a five-segment supply-demand function}\label{sec_example_5}
Here, we give an example of a five-segment supply-demand function. The number of time intervals is 24 and future prices are 78.92, 75.91, 70.9, 65.97, 62.4, 62.52, 62.77, 69.89, 73.58, 77.44, 77.98, 83.72, 82.24, 69.61, 61.1, 61.41, 61.45, 59.52, 59.66, 60.04, 61.87, 60.87, 61.91 (USD/MWh). The capacity of the battery is 22MWh, $\overline{P}=5$MW, $E_1=14$Mwh, and$\underline{E}$ and $\overline{E}$ are 0 and 22MWh (the setting of the battery is the same as Fig.\ref{fig:5seg}). Under these parameters, five segments are $P_{s1}$, $P_{s2}$, $P_{s3}^C$, $P_{s4}$ and $P_{s5}$. As for $P_{s1}$ and $P_{s5}$, they are fully charging and discharging segments. For $P_{s2}$, the value is -3MW, and the battery is fully charged at $t=8$ with $n_c=4$ and $n_d=3$. For $P_{s3}^C$, the value is -1MW, and the battery is fully discharged at $t=4$ with $n_c=0$ and $n_d=3$. For $P_{s4}$, the value is 4MW, and the battery is fully discharged at $t=3$ with $n_c=0$ and $n_d=2$.

\subsection{Model Generalization and demand-supply function}

\subsubsection{Different charging and discharging efficiencies and different charging and discharging maximums}
Denote $P^d_t$ and $P^c_t$ as the discharging and charging power at time $t$, $\overline{P^d}$ and $\overline{P^c}$ as the maximum discharging and charging power, and $\eta^d$ and $\eta^c$ as discharging and charging efficiencies. The objective function \eqref{eq:M1_1} in the base case changes to \eqref{eq:M1_EFF_OBJ}.
\begin{equation}\label{eq:M1_EFF_OBJ}
	M_1: \min_{\{P^d,P^c,E\}} \,\, J =\sum_{t=1}^{T}{-c_t (P^d_t-P^c_t) \Delta t}
\end{equation}	
Constraints \eqref{eq:M1_2} in the base case change to \eqref{eq:M1_EFF_1} and \eqref{eq:M1_EFF_3}; \eqref{eq:M1_3} in the base case  change to \eqref{eq:M1_EFF_4}:
\begin{equation}\label{eq:M1_EFF_1}
	(\underline{\alpha}^d_t, \ \overline{\alpha}^d_t):\ 0 \leq P^d_t \leq \overline{P^d}, \forall t 
\end{equation}			
\begin{equation}\label{eq:M1_EFF_2}
	(\underline{\alpha}^c_t, \ \overline{\alpha}^c_t):\ 0 \leq P^c_t \leq \overline{P^c}, \forall t
\end{equation}			
\begin{equation}\label{eq:M1_EFF_3}
	P^d_tP^c_t=0, \forall t 
\end{equation}
\begin{equation}\label{eq:M1_EFF_4}
	(\sigma_t):E_{t+1} = E_1 - \sum_{\tau=1}^{t}(\frac{P^d_\tau}{\eta^d} - P^c_\tau \eta^c)\Delta t, \forall t\in[2,T+1]
\end{equation}	

\par  Constraints (\ref{eq:M1_EFF_1}) and (\ref{eq:M1_EFF_2}) limit the upper and lower bounds of power; constraint (\ref{eq:M1_EFF_3}) limits that the storage system can not discharge and charge simultaneously at time $t$; constraint (\ref{eq:M1_EFF_4}) demonstrates the relationship between the stored energy at time $t+1$ considering the charging and discharging process before time $t+1$.




\subsubsection{Ending SOC limit}
%\textcolor{red}{Cong: emphasize the constraints and objective modification or replacement compare to Sec.10.2.1. If Fig.11  considers the energy dissipation, you can switch the sequence of Sec.10.2.3 and Sec.10.2.2.}


When the ending SOC is limited, the following equality constraint will be added
\begin{equation}\label{eq:M1_ENDSOC}
	(\mu):E_{T+1}=E_1 ,
\end{equation}		
which means the stored energy after the discharging and charging process should return to the initial value $E_1$. This may introduce two additional stairs corresponding to two new remainder energy levels. Please see Fig.\ref{fig:figy} as examples.

%The standard model tends to discharge energy to its lower bound since only the total profit is considered in the objective function. To address this issue, we can specify that the energy at time $T+1$ should be no lower than a given threshold, e.g., let $S_{T+1}\geq S_0$. 


\begin{figure}[H]
	\centering
	\includegraphics[width=2.0in]{pic/endingSOClimit.png}
	\caption{Impact of \textbf{the ending SOC limit} on the demand-supply functions of the energy storage system(the capacity is 2MWh, the maximum charging/discharging power is 0.6MW, the upper and lower bounds of SOC are 1 and 0.1, the initial SOC is 0.5, the total number of time periods is 24 with one time period being 1 hour) under extreme prices shown in Fig.\ref{fig:figx}(c). In (a) there are three kinds of stairs, which is the same as Fig.\ref{fig:figx}(f). In (b) there are seven kinds of stairs, and compared with Fig.\ref{fig:figx}(i) it can be observed that new discharging and charging stairs appear. In (c) there are six kinds of stairs, which is the same as Fig.\ref{fig:figx}(l).}
	\label{fig:figy}
\end{figure}
 


\subsubsection{Energy Dissipation}

%\textcolor{red}{Cong: emphasize the constraints and objective modification or replacement compare to Sec.10.2.1 or Sec.10.2.2}

When energy dissipation is considered, constraint (\ref{eq:M1_EFF_4}) changes to:
\begin{equation}\label{eq:M1_EFF_4}
	(\sigma_t):E_{t+1} = (1-\epsilon)^t E_1 - \sum_{\tau=1}^{t}(1-\epsilon)^{t-\tau}(\frac{P^d_\tau}{\eta^d} - P^c_\tau \eta^c)\Delta t, \forall t\in[2,T+1],
\end{equation}	
where $\epsilon$ denotes the dissipation rate of the battery.


%\subsubsection{Different charging and discharging maximum capacity limits}




\section{Supplemental Materials}

\textcolor{red}{May be we will show the most complicated complete model here first and explain the generalization to all these cases one by one.}

\subsection{Relaxation of $M1$}
We define the model with (\ref{eq:s}) relaxed, i.e., removed from $M1$, as $M2$. The sufficient condition for the exact relaxation is proposed and proved in this subsection.
\begin{theorem}\label{thm1}
	\textit{Assume $c_t>0$ holds for $\forall t$, the optimal solutions of decision variables in $M2$ is also optimal for $M1$.}
\end{theorem}

\par Proof of Theorem \ref{thm1} can be found in Appendix \ref{secA1}. The exactness of the $M2$ can be interpreted intuitively: with $c_t>0$ satisfied, charging and discharging simultaneously will waste energy. It is uneconomic for a storage system since the wasted energy should be charged back with $c_t$ which increases the cost. Therefore, the optimal solution in $M2$ still implicitly satisfies the constraint (\ref{eq:s}). 


\begin{theorem}\label{thm2}
	\textit{Assume there exists a feasible solution for M2. The function of the demand-supply function $P_1=f(c_1)$ is staircase and monotonically non-decreasing.}
\end{theorem}
Proof of Theorem \ref{thm2} can be found in Appendix \ref{secA2}.



\par The time interval at which $E_t$ is bound by an equality equation for the first time is defined as $T^B+1$. The equality equation can be $E_{T^B+1}=\underline{E}$, $E_{T^B+1}=\overline{E}$ and $E_{T^B+1}=E_1$. $n_c$ is defined as the number of time intervals when $P_t=\overline{P^c}, t\leq T^B$; $n_d$ is defined as the number of time intervals when $P_t=\overline{P^d}, t\leq T^B$; $n_0$ is defined as the number of time intervals when $P_t=0, t\leq T^B$.

\begin{lemma}\label{lem1}
	\textit{There exists an optimal solution of $M2$ which satisfies $T^B-n_c-n_d-n_0\leq1$.} 
\end{lemma}
Proof of Lemma \ref{lem1} can be found in Appendix \ref{secA3}.


\begin{theorem}\label{thm3}
\textit{When parameters of $\{E_1$, $c$, $\eta^d$, $\eta^c$, $T$, $\underline{E}$, $\overline{E}$, $\overline{P^d}$, $\overline{P^c}\}$ are given, the number of kinds of segments in the demand-supply functions is no more than 9.}
\end{theorem}
Proof of Theorem \ref{thm3} can be found in Appendix \ref{secA4}.

\subsection{Parameter Sensitivities}

Formally presented by the following theorem:

\begin{theorem}
    Consider a battery whose decision model is presented in (M1). For any point ($c_1$,$P_1$) on its original supply-demand curve, there exists an $\alpha$ such that the point ($c_1+\alpha$,$P_1$) is on its new curve when its future price forecast changes to $c_2'...c_T'$ and all other quantities do not change, and there exists an $\beta$ such that the point ($c_1$,$P_1+\beta$) is on its new curve when its initial SOC $E_1$ changes to $E_1'$ and all other quantities do not change.
\end{theorem}


==> method_v0_2.tex <==
\section{Methods}

In this method section, we first provide the base case and the proof of its demand-supply function. Then, we provide generalizations considering battery efficiencies, energy dissipation, and the ending SOC limit. Detailed proofs of the generalized demand-supply functions are provided in the supplemental material.

\subsection{Model used to generate the demand-supply function}
\subsubsection{Battery opportunity cost minimization}
To generate the demand-supply function of a battery, the following multi-period look-ahead optimization model is adopted as our basic model:
\begin{equation}\label{eq:M1_1}
	M_1: \min_{\{P,E\}} \,\, J =\sum_{t=1}^{T}{-c_t P_t \Delta t}
\end{equation}	
subject to the following constraints for 
\begin{equation}\label{eq:M1_2}
	(\underline{\alpha}_t, \ \overline{\alpha}_t):\ -\overline{P} \leq P_t \leq \overline{P} ,\forall t \in [1,T]
\end{equation}			
%\begin{equation}\label{eq:M1_3}
%	(\underline{\alpha}^c_t, \ \overline{\alpha}^c_t):\ 0 \leq P^c_t \leq \overline{P^c}
%\end{equation}			
%\begin{equation}\label{eq:s}
%	P^d_tP^c_t=0 
%\end{equation}
\begin{equation}\label{eq:M1_3}
	(\sigma_t):E_{t+1} = E_1 - \sum_{\tau=1}^{t} P_\tau  \Delta t,\forall t \in [1,T]
\end{equation}	
\begin{equation}\label{eq:M1_4}
	(\underline{\beta}_t, \ \overline{\beta}_t):\ \underline{E} \leq E_{t} \leq \overline{E} ,\forall t \in [2,T+1]
\end{equation}			
where $c_t$ is the electricity price at time $t$; $P_t$ is the net power output of the battery, for which positive means discharging and negative means charging. $E_t$ is the stored energy at time $t$ before the discharging and charging process at time $t$; \textcolor{red}{$T$ is the number of time intervals in one day and $\Delta t$ is the time length of one single interval, i.e. $\Delta t = (24~\text{hour})/T$}; $\overline{P}$ is the maximum discharging and charging power; $\overline{E}$ and $\underline{E}$ are the upper and lower limits of the stored energy; $E_1$ is the initial stored energy; $\underline{\alpha}_t$  and  $\overline{\alpha}_t$ are the multipliers of constraint \eqref{eq:M1_2}; $\sigma_t$ is the multiplier of constraint \eqref{eq:M1_3}; $\underline{\beta}_t$  and  $\overline{\beta}_t$ are the multipliers of constraint \eqref{eq:M1_4}. 

\par The objective in (\ref{eq:M1_1}) is the total cost of storage systems in one day. Constraints (\ref{eq:M1_2})  limit the upper and lower bounds of power;  constraint (\ref{eq:M1_3}) demonstrates the relationship between the stored energy at time $t+1$ considering the charging and discharging process before time $t+1$; constraint (\ref{eq:M1_4}) limits the upper and lower bounds of the stored energy.


\subsubsection{Demand-supply function and Proof of Theorem \ref{BaseCaseTHM}}
The model in \eqref{eq:M1_1} is standard and widely adopted in the literature \cite{davies2019combined, ransan2021applying, beuse2021comparing, qin2023role, JiangPowell15Storage, Lamadrid24JRE, Alshehri&etal:20TPS, attarha23TEMPR}. Given a set of battery parameters, future price forecast $c_2, ...c_T$, and an initial SOC $E_1$, we solve the optimal charging and discharging power with different prices for the current interval $c_1$ and formulate $P_1$ as a function of $c_1$. Such a function $P_1=f(c_1)$ is exactly the demand-supply function we study in this paper.

In Fig.~\ref{fig:5seg}, we provide the five-segment example for the demand-supply function of the battery, supported by Theorem \ref{BaseCaseTHM}. Here we first provide the Lemma~\ref{BaseCaseN1less},  Lemma~\ref{BaseCaselemma3}, and Lemma~\ref{BaseCaselemma2}. Then we finish the proof of Theorem \ref{BaseCaseTHM}.

%\textcolor{red}{Could you finish the proof below with the simplified base case model (1)-(4)?}

Denote $T^B+1$ as the first time we have the binding inequality constraint \eqref{eq:M1_4}, $n_c$ as the number of intervals when $P_t=-\overline{P}, \forall t \leq T^B$,  and $n_d$ as the number of intervals when $P_t=\overline{P}, \forall t \leq T^B$. Denote $j$ as the time index  when $-\overline{P} < P_j < \overline{P}$ and  $j\le T^B$. An example of these terms is shown in Fig.\ref{fig:denotation_of_terms}.
\begin{figure}[h]
	\centering
	\includegraphics[width=3.5in]{pic/denotation of terms.png}
	\caption{An example of battery action trajectory with black curves for discharging and green curves for charging. Notations $T^B+1$, $n_c$, $n_d$, and $j$ are marked.}
	\label{fig:denotation_of_terms}
\end{figure}

\newtheorem{lemma}{Lemma}
\begin{lemma}\label{BaseCaseN1less}
	\textit{There exists an optimal solution of $M_1$ satisfying $T^B-n_c-n_d\leq1$.} 
\end{lemma}
\begin{proof}[Proof of Lemma~{\upshape\ref{BaseCaseN1less}}]
	
We prove this lemma by contradiction. Suppose there exist more than one time interval such that $-\overline{P} < P_t < \overline{P}$, i.e. $\Omega:=\{t\le T^B|-\overline{P} < P_t < \overline{P}\}$, and $N:=|\Omega|, N>1$. From the KKT condition of $M_1$, we have:
%$\rho_t=\sum_{t'=t}^{T^B} (\underline{\beta}-\overline{\beta})$.
\begin{align}
    &\frac{\partial L}{\partial P_t} = -c_t \Delta t - \underline{\alpha_t} + \overline{\alpha_t} + \sum_{\tau\geq t}{\sigma_{\tau} \Delta t} = 0, \ \forall t \in [1,T]. \label{eq:omegaKKT_P} \\
    &\frac{\partial L}{\partial E_t} = \sigma_{t-1} -\underline{\beta}_t + \overline{\beta}_t= 0, \ \forall t \in [2,T+1]. \label{eq:omegaKKT_E}
\end{align}
\par Since $T^B+1$ is the first time interval when the inequality constraint \eqref{eq:M1_4} is binding, $\underline{\beta_t}= \overline{\beta_t}=0, \forall t\le T^B$ in \eqref{eq:omegaKKT_E}. Therefore, $\sigma_t =0, \forall t\le T^B$ and  $\underline{\alpha}_t=\overline{\alpha}_t=0, \forall t\in \Omega$. Substituting these into \eqref{eq:omegaKKT_P}, we have
\begin{equation}\label{eq:omegaKKT_P_omega}
    \frac{\partial L}{\partial P_t} = -c_t \Delta t + \sigma_{T^B} \Delta t = 0, \ \forall t \in \Omega. \Rightarrow c_t=\sigma_{T^B}, \forall t\in \Omega.
\end{equation}
%Therefore, $c_t=\sigma_{T^B}, \forall t\in \Omega$. 
    %-c^n \sum_{t \in T^n} P_t \Delta t = \mu (\sum_{t \in T^n} P_t \Delta t)
% that satisfying the objective function and all constraints, i.e. $\sum_{t \in \Omega} \hat{P}_t \Delta t = \sum_{t \in \Omega} P_t \Delta t$.
\par Denote $N':=\lfloor{\frac{|\sum_{t \in \Omega} P_t|}{\overline{P}}}\rfloor$. We have %$N' \overline{P}\leq |\sum_{t \in \Omega} P_t| < (N'+1)\overline{P}$. Then the following equations can be derived:
\begin{align}
    N' \overline{P}\leq |\sum_{t \in \Omega} P_t| < (N'+1)\overline{P} \Rightarrow \begin{subequations}
        \begin{cases}\label{eq:lem1N'le0}
            0 \leq  -N' \overline{P}+ \sum_{t \in \Omega} P_t < \overline{P},  &\sum_{t \in \Omega} P_t  \geq 0, \\ %\label{eq:lem1N'ge0} \\
            -\overline{P} < N' \overline{P}+ \sum_{t \in \Omega} P_t\leq 0,  &\sum_{t \in \Omega} P_t  \leq 0. %\label{eq:lem1N'le0}
        \end{cases}
    \end{subequations}
\end{align}
We define $\{\hat{P}_t\}_{t \in \Omega}$ by the following four cases:
In all four cases, the time indexes in $\Omega$ are renumbered from $j$ to $j+N-1$ according to the original order, with $j$ being the first element.
\begin{itemize}
    \item \underline{Case1: $N=N'+2n$ for some integer $n$. }
    \begin{itemize}
        \item \underline{Case1.A ($\sum_{t \in \Omega} P_t\geq 0$):}  
        $\hat{P}_j= -(N'+1) \overline{P}+\sum_{t \in \Omega} P_t$ and by definition, $j$ is the smallest time index in $\Omega$. Add $-\overline{P}$ to both sides of \eqref{eq:lem1N'le0}, we have
            \begin{equation}
                -\overline{P} \leq -(N'+1) \overline{P}+ \sum_{t \in \Omega} P_t< 0 \Rightarrow \hat{P}_j \in [-\overline{P}, 0).
            \end{equation} 
            
            For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, $\hat{P}_t =\overline{P}, \forall t=\{j+1,j+3,...,j+2n-3,j+N-N'-1,..,j+N-1\}$, otherwise, $ \hat{P}_t =-\overline{P}$.
            
            %\textcolor{red}{For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, for the smallest $2n-2$ time indexes in $\Omega$ except $j$, $\overline{P}$ and $-\overline{P}$ are set by turns according the order of the time index; for the largest $N'+1$ time indexes, $\overline{P}$ are set. (Cong: try $ \hat{P}_t =\overline{P}, \forall t=\{j+1,... \}$, otherwise, $ \hat{P}_t =-\overline{P}$. You can renumber the time indexes in $\Omega$ saying $j$ is the first element.}%\textcolor{red}{For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, we randomly assign $N'+n$ of them to be $\overline{P}$ and $n-1$ of them to be $-\overline{P}$. According to Cong: I notice that we cannot randomly assign, we need to make it satisfy the SoC limit constraints. Could you provide the assigning details that satisfy the constraint?}% \textcolor{red}{Cong's revision: did you show that ?} %\textcolor{red}{; Cong: you need to specify which $\hat{P}_t$ is $\overline{P}$ and which one goes to $-\overline{P}$. Define $\{\hat{P}_t\}_{t \in \Omega}$ precisely. Similar modifications are needed for all other cases.}
        \item \underline{Case1.B ($\sum_{t \in \Omega} P_t\leq 0$):} $\hat{P}_j= (N'+1) \overline{P}+\sum_{t \in \Omega} P_t$. Add $\overline{P}$ to both sides of \eqref{eq:lem1N'le0}, we have
            \begin{equation}
                0 < -(N'+1) \overline{P}+ \sum_{t \in \Omega} P_t \leq \overline{P} \Rightarrow \hat{P}_j \in (0, \overline{P}].
            \end{equation} 
        For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, $\hat{P}_t =-\overline{P}, \forall t=\{j+1,j+3,...,j+2n-3,j+N-N'-1,..,j+N-1\}$, otherwise, $ \hat{P}_t =\overline{P}$.
    \end{itemize}
    \item \underline{Case2:  $N=N'+2n+1$ for some integer $n$. }
    \begin{itemize}
        \item \underline{Case2.A ($\sum_{t \in \Omega} P_t\geq 0$):} 
        $\hat{P}_j= -N' \overline{P}+\sum_{t \in \Omega} P_t$. According to \eqref{eq:lem1N'le0}, we have
            \begin{equation}
                \hat{P}_j \in [0,\overline{P}).
            \end{equation} 
            For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, $\hat{P}_t =\overline{P}, \forall t=\{j+2,j+4,...,j+2n,j+N-N',..,j+N-1\}$, otherwise, $ \hat{P}_t =-\overline{P}$.
        \item \underline{Case2.B ($\sum_{t \in \Omega} P_t\leq 0$):} 
        $\hat{P}_j= N' \overline{P}+\sum_{t \in \Omega} P_t$. According to \eqref{eq:lem1N'le0}, we have 
            \begin{equation}
                \hat{P}_j \in (-\overline{P},0].
            \end{equation} 
        For $\{\hat{P}_t\}_{t\in \Omega, t\neq j}$, $\hat{P}_t =-\overline{P}, \forall t=\{j+2,j+4,...,j+2n,j+N-N',..,j+N-1\}$, otherwise, $ \hat{P}_t =\overline{P}$.
    \end{itemize}
\end{itemize}
 % $\hat{P}_t, t \in \Omega$
For $\{\hat{P}_t\}_{t \in \Omega}$, we can easily show that (i) $\hat{\Omega}:=\{t\le T^B|-\overline{P} < \hat{P}_t < \overline{P}\}$, $|\hat{\Omega}|\le 1$; (ii) $\hat{P}_t, t \in \Omega$ is an equal optimal solution to $P_t, t \in \Omega$ because they achieve the same objective value and satisfy all constraints. For the objective value, according to \eqref{eq:omegaKKT_P_omega}, we have $\sum_{t\in \Omega}{c_tP_t}= \sigma_{T^B} \sum_{t\in \Omega}{P_t}$. And by the definition of $\{\hat{P}_t\}_{t \in \Omega}$, we have $\sum_{t\in \Omega}{P_t} = \sum_{t\in \Omega}{\hat{P}_t}$. Therefore, the objective function is the same. For constraints, the definition of $\{\hat{P}_t\}_{t \in \Omega}$ will not let the battery be fully charged or discharged before $T^B+1$, which results in satisfying constraint \eqref{eq:M1_4}. And according to the definition of $\{\hat{P}_t\}_{t \in \Omega}$, constraint \eqref{eq:M1_2} holds. And since we have $\sum_{t\in \Omega}{P_t} = \sum_{t\in \Omega}{\hat{P}_t}$, constraint \eqref{eq:M1_3} holds. 

% By analyzing all possible cases of $\hat{P}_t, t \in \Omega$, $\hat{\Omega}:=\{t\le T^B|-\overline{P} < \hat{P}_t < \overline{P}\}$, $|\hat{\Omega}|\le 1$. hat satisfying the objective function and all constraints, 
Therefore, it is always possible to find an optimal solution that $T^B-n_c-n_d\leq1$ holds.
\end{proof} 



\begin{lemma}\label{BaseCaselemma3}
	\textit{The demand-supply function of an ideal battery is a staircase monotonic non-decreasing function.} 
\end{lemma}
\begin{proof}[Proof of Lemma~{\upshape\ref{BaseCaselemma3}}]
    \par First, by utilizing the properties of multi-parametric linear programming, a proof of the staircase property is conducted. The dual problem of $M_1$ is as follows: 
    \begin{equation}
        M_{1,\text{(dual)}}:  \min_{u} \, W = b'u 
    \end{equation}   
    subject to
    \begin{equation}
        (P): \, G'u \leq c 
    \end{equation}
    According to the properties of the multi-parametric linear programming problem (MPLP) (Theorem 6.5 in \cite{borrelli2017predictive}), for $M_{1,\text{(dual)}}$, the function $W^*(c)$ is a piecewise affine convex function (with the electricity price $c$ as a parameter). Therefore, the function $P(c) = \frac{\partial W^*(c)}{\partial c}$ is a stepwise monotonic non-decreasing function.
\end{proof}



\begin{lemma}\label{BaseCaselemma2}
	\textit{Given the parameters $\{E_1, c, T, \underline{E}, \overline{E}, \overline{P}\}$, if for $M_1$ there exists $T^B$ such that $E_{T^B+1} = \underline{E}$, then as $c_1$ increases, there will be no $T^B$ such that $E_{T^B+1} = \overline{E}$ holds.
} 
\end{lemma}
\begin{proof}[Proof of Lemma~{\upshape\ref{BaseCaselemma2}}]
$M_3$ can be regarded as the problem of finding the optimal solution for times $t = 2$ to $T$, given that the optimal solution at $t = 1$ is known. When $\{E_1, c, T, \underline{E}, \overline{E}, \overline{P}\}$ remain unchanged, the optimal solution of $M_3$ is optimal in $M_1$. Based on the non-decreasing characteristic of the energy storage supply-demand function, as $c_1$ increases shown in Lemma.\ref{BaseCaselemma3}, $P_1$ either remains unchanged or increases, resulting in the energy consumption at $t=1$ remaining unchanged or increasing. Therefore, $E_2$, i.e. the initial energy storage level in $M_3$, remains unchanged or decreases. Suppose there originally existed $T^B$ such that $E_{T^B+1} = \underline{E}$, when other parameters remain unchanged and $E_2$ remains unchanged, the energy in the battery will be fully discharged at $T^B+1$; when $E_2$ decreases, the energy in the battery will be fully discharged at $T^B+1$ or before $T^B+1$. In any of these cases, the battery will not be fully charged before it has been fully discharged. Therefore, there will not exist a $T^B$ such that $E_{T^B+1} = \overline{E}$.
\end{proof}


\begin{proof}[Proof of Theorem~{\upshape\ref{BaseCaseTHM}}]
We below prove that, for the optimal solution of the model $M_1$, $P^*_{1}\in \{P_{s1}, P_{s2}  P_{s3}^C, P_{s3}^d, P_{s4}, P_{s5}\}$ and there are at most 5 segments existing simultaneously. 
% \textcolor{blue}{ \begin{equation}
%          P_1(c_1)=\begin{cases} -\overline{P},& \text{if}~ c_1\le c_1^a,\\
%          \frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P},& \text{if}~ c_1^a < c_1\le  c_1^b,\\
%          \frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}~\text{or}~ \frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P},& \text{if}~ c_1^b < c_1\le  c_1^c,\\
%          \frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P},& \text{if}~ c_1^c< c_1 \le c_1^d,\\
%          \overline{P},& \text{if}~ c_1\ge  c_1^d,\\
%      \end{cases}
%  \end{equation}
%  where $n_d$ and $n_c$ are functions of $c_1$.}
 
%From Lemma~\ref{BaseCaseN1less},  $j \in \{\emptyset,1, 2, ..., T^B\}$.

	\par \underline{Case1 ($T^B-n_c-n_d=0$ or $T^B-n_c-n_d=1, j\neq 1$):} Denote the fully-charge by $P_{s1}=-\overline{P}$ and the fully-discharge segments by $P_{s5}=\overline{P}$. In this case, from Lemma~\ref{BaseCaseN1less}, $P_{1}\in \{P_{s1}, P_{s5}\}$.


% \textcolor{blue}{Denote $c_1^d$ be the value such that $T^B-n_c-n_d=1, j=1$.}
    \par \underline{Case2 ($T^B-n_c-n_d=1, j=1$):}   \begin{align}
    \begin{aligned}
        &E_{T^B+1} \overset{(a)}{=} E_1 - \sum_{\tau=1}^{t} P_\tau  \Delta t \overset{(b)}{=} E_1 - (n_d - n_c)\overline{P}+ P_{1}, \\
         \overset{(c)}{\Rightarrow} &P_{1} = \frac{E_1 - E_{T^B+1}}{\Delta t} - (n_d - n_c)\overline{P}.\label{eq:Theorem1_1}
        \end{aligned}
    \end{align} 
    where (a) comes from  (\ref{eq:M1_3}); (b) comes from the definition of $n_d, n_c$, $P_1 \in (-\overline{P}, \overline{P})$ from the definition of $j$, and   $P_t \in \{-\overline{P}, \overline{P}\}, \forall 2\le t \le T^B$ from Lemma~\ref{BaseCaseN1less};   (c) is derived by moving elements around the equation.
    
%    According to Lemma~\ref{BaseCaseN1less} and (\ref{eq:M1_3}),
	%\begin{equation}\label{eq:Theorem1_1}
%		P_{1} = \frac{E_1 - E_{T^B+1}}{\Delta t} - (n_d - n_c)\overline{P}
%	\end{equation}
%	holds. 
Four segments can be derived by \eqref{eq:Theorem1_1}: 
    \begin{itemize}
         \item  When $P_{1}\leq 0$, \begin{cases}
             P_{s2}=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P},\text{the Charge-for-charge segment}, \\
             P_{s3}^C=\frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}, \text{the Charge-for-discharge segment}.
         \end{cases}
         \item  When $P_{1}\geq 0$, \begin{cases} P_{s3}^D=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P}$, \text{the Discharge-for-charge segment},\\
          P_{s4}=\frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}$,  \text{the Discharge-for-discharge segment}.
         \end{cases} 
    \end{itemize}
    \par Note that according to constraints \eqref{eq:M1_2}, we have:
    \begin{align}
        -\overline{P}&<P_{s2}\leq 0 \label{eq:the1_ncnd_ps2} \\
        -\overline{P}&<P_{s3}^C\leq 0 \label{eq:the1_ncnd_ps3C} \\
        0&\leq P_{s3}^D < \overline{P} \label{eq:the1_ncnd_ps3D} \\
        0&\leq P_{s4}< \overline{P} \label{eq:the1_ncnd_ps4} 
    \end{align}
    Then by substituting $P_{s2}=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P}$ into \eqref{eq:the1_ncnd_ps2}, we have \eqref{eq:the1_ncnd_ps2_re}; by substituting $P_{s3}^C=\frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}$ into \eqref{eq:the1_ncnd_ps3C}, we have \eqref{eq:the1_ncnd_ps3C_re}; by substituting $P_{s3}^D=\frac{E_1 - \overline{E}}{\Delta t} - (n_d - n_c)\overline{P}$ into \eqref{eq:the1_ncnd_ps3D}, we have \eqref{eq:the1_ncnd_ps3D_re}; by substituting $P_{s4}=\frac{E_1 - \underline{E}}{\Delta t} - (n_d - n_c)\overline{P}$ into \eqref{eq:the1_ncnd_ps4}, we have \eqref{eq:the1_ncnd_ps4_re}.
    \begin{align}
        &\text{for} P_{s2}: \frac{E_1-\overline{E}}{\overline{P} \Delta t} \leq n_d-n_c <\frac{E_1-\overline{E}}{\overline{P}\Delta t} +1 \label{eq:the1_ncnd_ps2_re} \\
        &\text{for} P_{s3}^C: \frac{E_1-\underline{E}}{\overline{P} \Delta t} \leq n_d-n_c <\frac{E_1-\underline{E}}{\overline{P}\Delta t} +1 \label{eq:the1_ncnd_ps3C_re} \\
        &\text{for} P_{s3}^D: \frac{E_1-\overline{E}}{\overline{P} \Delta t} -1 < n_d-n_c \leq \frac{E_1-\overline{E}}{\overline{P}\Delta t} \label{eq:the1_ncnd_ps3D_re} \\
        &\text{for} P_{s4}: \frac{E_1-\underline{E}}{\overline{P} \Delta t} -1 < n_d-n_c \leq \frac{E_1-\underline{E}}{\overline{P}\Delta t} \label{eq:the1_ncnd_ps4_re} 
    \end{align}
    Here, if we denote $\frac{E_1-\overline{E}}{\overline{P} \Delta t}$ as $K$, we have $K \leq n_d-n_c<K+1$. Since $n_d-n_c$ is an integer, for \eqref{eq:the1_ncnd_ps2_re} only one value exists for $n_d-n_c$. Similarly, for \eqref{eq:the1_ncnd_ps3C_re}, \eqref{eq:the1_ncnd_ps3D_re} and \eqref{eq:the1_ncnd_ps4_re}, there exists only one $n_d-n_c$ for each of them. %\textcolor{red}{Cong: You only show $P_s2$-$P_s4$ are four constants. Did you show that $P_s2$-$P_s4$ are different values?} \textcolor{purple}{Chenge: Sometimes, values of $P_{s2}$ and $P_{s3}^C$ are equal, values of $P_{s4}$ and $P_{s3}^D$ are equal. For example when Emax=20MWh, Emin=0, Pmax=5MW, E1=12.5MWh. We have $P_{s2}=P_{s3}^C=-2.5$ and $P_{s4}=P_{s3}^D=2.5$. Therefore, the values of stairs may be equal. I've tried, but proving that $P_s2$-$P_s4$ are different values is difficult. Now we have different functions of them, do you think it is enough?}  
    Therefore,  $P_{s2}$, $P_{s3}^C$, $P_{s3}^D$, and $P_{s4}$ are four constants. %\textcolor{red}{It is noted that there exists at most one value of $n_d-n_c$ for each of \eqref{eq:the1_ncnd_ps2_re}-\eqref{eq:the1_ncnd_ps4_re}.  Cong: how can you see this? D you need to prove like for $P_{s4}$, the gap between upper and lower bounds has $ k-1 < \frac{E_1-\underline{E}}{\overline{P}\Delta t} - \frac{E_1-\underline{E}}{\overline{P} \Delta t} < k+1$?} 
%    In Fig.XX, we present the example with all four different constants, construct four . }    
    \par Until now we prove six constants $P_{s1}$, $P_{s2}$, $P_{s3}^C$, $P_{s3}^D$,  $P_{s4}$, and $P_{s5}$ constructing the segments in the stair functions $P_1(c_1)$. According to Lemma~\ref{BaseCaselemma2}, $P_{s3}^C$ and $P_{s4}^D$ can not appears simultaneously.  In Sec.\ref{sec_example_5}, we present an example with five segments exist. Therefore, the total number of segments is at most five. %And when no $n_d-n_c$ satisfies any of \eqref{eq:the1_ncnd_ps2_re}-\eqref{eq:the1_ncnd_ps4_re}, corresponding segments $P_{s2}$, $P_{s3}^C$, $P_{s3}^D$, and $P_{s4}$ will not exist. And if the initial SOC is not enough for fully charging or discharging for one time interval, the corresponding fully charge segment $P_{s1}$ or fully discharge segment $P_{s5}$ will not exist. Therefore, the total number of segments is at most 5.  
\end{proof}	 

\subsubsection{An example of a five-segment supply-demand function}\label{sec_example_5}
\textcolor{red}{Modify later with a shorter time horizon and table showing all data.}

Here, we give an example of a five-segment supply-demand function. The number of time intervals is 24 and future prices are 78.92, 75.91, 70.9, 65.97, 62.4, 62.52, 62.77, 69.89, 73.58, 77.44, 77.98, 83.72, 82.24, 69.61, 61.1, 61.41, 61.45, 59.52, 59.66, 60.04, 61.87, 60.87, 61.91 (USD/MWh). The capacity of the battery is 22MWh, $\overline{P}=5$MW, $E_1=14$Mwh, and$\underline{E}$ and $\overline{E}$ are 0 and 22MWh (the setting of the battery is the same as Fig.\ref{fig:5seg}). Under these parameters, five segments are $P_{s1}$, $P_{s2}$, $P_{s3}^C$, $P_{s4}$ and $P_{s5}$. As for $P_{s1}$ and $P_{s5}$, they are fully charging and discharging segments. For $P_{s2}$, the value is -3MW, and the battery is fully charged at $t=8$ with $n_c=4$ and $n_d=3$. For $P_{s3}^C$, the value is -1MW, and the battery is fully discharged at $t=4$ with $n_c=0$ and $n_d=3$. For $P_{s4}$, the value is 4MW, and the battery is fully discharged at $t=3$ with $n_c=0$ and $n_d=2$.

\subsection{Model Generalization and demand-supply function}

\subsubsection{Different charging and discharging efficiencies and different charging and discharging maximums}
Denote $P^d_t$ and $P^c_t$ as the discharging and charging power at time $t$, $\overline{P^d}$ and $\overline{P^c}$ as the maximum discharging and charging power, and $\eta^d$ and $\eta^c$ as discharging and charging efficiencies. The objective function \eqref{eq:M1_1} in the base case changes to \eqref{eq:M1_EFF_OBJ}.
\begin{equation}\label{eq:M1_EFF_OBJ}
	M_1: \min_{\{P^d,P^c,E\}} \,\, J =\sum_{t=1}^{T}{-c_t (P^d_t-P^c_t) \Delta t}
\end{equation}	
Constraints \eqref{eq:M1_2} in the base case change to \eqref{eq:M1_EFF_1} and \eqref{eq:M1_EFF_3}; \eqref{eq:M1_3} in the base case  change to \eqref{eq:M1_EFF_4}:
\begin{equation}\label{eq:M1_EFF_1}
	(\underline{\alpha}^d_t, \ \overline{\alpha}^d_t):\ 0 \leq P^d_t \leq \overline{P^d}, \forall t 
\end{equation}			
\begin{equation}\label{eq:M1_EFF_2}
	(\underline{\alpha}^c_t, \ \overline{\alpha}^c_t):\ 0 \leq P^c_t \leq \overline{P^c}, \forall t
\end{equation}			
\begin{equation}\label{eq:M1_EFF_3}
	P^d_tP^c_t=0, \forall t 
\end{equation}
\begin{equation}\label{eq:M1_EFF_4}
	(\sigma_t):E_{t+1} = E_1 - \sum_{\tau=1}^{t}(\frac{P^d_\tau}{\eta^d} - P^c_\tau \eta^c)\Delta t, \forall t\in[2,T+1]
\end{equation}	

\par  Constraints (\ref{eq:M1_EFF_1}) and (\ref{eq:M1_EFF_2}) limit the upper and lower bounds of power; constraint (\ref{eq:M1_EFF_3}) limits that the storage system can not discharge and charge simultaneously at time $t$; constraint (\ref{eq:M1_EFF_4}) demonstrates the relationship between the stored energy at time $t+1$ considering the charging and discharging process before time $t+1$.




\subsubsection{Ending SOC limit}
%\textcolor{red}{Cong: emphasize the constraints and objective modification or replacement compare to Sec.10.2.1. If Fig.11  considers the energy dissipation, you can switch the sequence of Sec.10.2.3 and Sec.10.2.2.}


When the ending SOC is limited, the following equality constraint will be added
\begin{equation}\label{eq:M1_ENDSOC}
	(\mu):E_{T+1}=E_1 ,
\end{equation}		
which means the stored energy after the discharging and charging process should return to the initial value $E_1$. This may introduce two additional stairs corresponding to two new remainder energy levels. Please see Fig.\ref{fig:figy} as examples.

%The standard model tends to discharge energy to its lower bound since only the total profit is considered in the objective function. To address this issue, we can specify that the energy at time $T+1$ should be no lower than a given threshold, e.g., let $S_{T+1}\geq S_0$. 


\begin{figure}[H]
	\centering
	\includegraphics[width=2.0in]{pic/endingSOClimit.png}
	\caption{Impact of \textbf{the ending SOC limit} on the demand-supply functions of the energy storage system(the capacity is 2MWh, the maximum charging/discharging power is 0.6MW, the upper and lower bounds of SOC are 1 and 0.1, the initial SOC is 0.5, the total number of time periods is 24 with one time period being 1 hour) under extreme prices shown in Fig.\ref{fig:figx}(c). In (a) there are three kinds of stairs, which is the same as Fig.\ref{fig:figx}(f). In (b) there are seven kinds of stairs, and compared with Fig.\ref{fig:figx}(i) it can be observed that new discharging and charging stairs appear. In (c) there are six kinds of stairs, which is the same as Fig.\ref{fig:figx}(l).}
	\label{fig:figy}
\end{figure}
 


\subsubsection{Energy Dissipation}

%\textcolor{red}{Cong: emphasize the constraints and objective modification or replacement compare to Sec.10.2.1 or Sec.10.2.2}

When energy dissipation is considered, constraint (\ref{eq:M1_EFF_4}) changes to:
\begin{equation}\label{eq:M1_EFF_4}
	(\sigma_t):E_{t+1} = (1-\epsilon)^t E_1 - \sum_{\tau=1}^{t}(1-\epsilon)^{t-\tau}(\frac{P^d_\tau}{\eta^d} - P^c_\tau \eta^c)\Delta t, \forall t\in[2,T+1],
\end{equation}	
where $\epsilon$ denotes the dissipation rate of the battery.


%\subsubsection{Different charging and discharging maximum capacity limits}




\section{Supplemental Materials}

\textcolor{red}{May be we will show the most complicated complete model here first and explain the generalization to all these cases one by one.}

\subsection{Relaxation of $M1$}
We define the model with (\ref{eq:s}) relaxed, i.e., removed from $M1$, as $M2$. The sufficient condition for the exact relaxation is proposed and proved in this subsection.
\begin{theorem}\label{thm1}
	\textit{Assume $c_t>0$ holds for $\forall t$, the optimal solutions of decision variables in $M2$ is also optimal for $M1$.}
\end{theorem}

\par Proof of Theorem \ref{thm1} can be found in Appendix \ref{secA1}. The exactness of the $M2$ can be interpreted intuitively: with $c_t>0$ satisfied, charging and discharging simultaneously will waste energy. It is uneconomic for a storage system since the wasted energy should be charged back with $c_t$ which increases the cost. Therefore, the optimal solution in $M2$ still implicitly satisfies the constraint (\ref{eq:s}). 


\begin{theorem}\label{thm2}
	\textit{Assume there exists a feasible solution for M2. The function of the demand-supply function $P_1=f(c_1)$ is staircase and monotonically non-decreasing.}
\end{theorem}
Proof of Theorem \ref{thm2} can be found in Appendix \ref{secA2}.



\par The time interval at which $E_t$ is bound by an equality equation for the first time is defined as $T^B+1$. The equality equation can be $E_{T^B+1}=\underline{E}$, $E_{T^B+1}=\overline{E}$ and $E_{T^B+1}=E_1$. $n_c$ is defined as the number of time intervals when $P_t=\overline{P^c}, t\leq T^B$; $n_d$ is defined as the number of time intervals when $P_t=\overline{P^d}, t\leq T^B$; $n_0$ is defined as the number of time intervals when $P_t=0, t\leq T^B$.

\begin{lemma}\label{lem1}
	\textit{There exists an optimal solution of $M2$ which satisfies $T^B-n_c-n_d-n_0\leq1$.} 
\end{lemma}
Proof of Lemma \ref{lem1} can be found in Appendix \ref{secA3}.


\begin{theorem}\label{thm3}
\textit{When parameters of $\{E_1$, $c$, $\eta^d$, $\eta^c$, $T$, $\underline{E}$, $\overline{E}$, $\overline{P^d}$, $\overline{P^c}\}$ are given, the number of kinds of segments in the demand-supply functions is no more than 9.}
\end{theorem}
Proof of Theorem \ref{thm3} can be found in Appendix \ref{secA4}.

\subsection{Parameter Sensitivities}

Formally presented by the following theorem:

\begin{theorem}
    Consider a battery whose decision model is presented in (M1). For any point ($c_1$,$P_1$) on its original supply-demand curve, there exists an $\alpha$ such that the point ($c_1+\alpha$,$P_1$) is on its new curve when its future price forecast changes to $c_2'...c_T'$ and all other quantities do not change, and there exists an $\beta$ such that the point ($c_1$,$P_1+\beta$) is on its new curve when its initial SOC $E_1$ changes to $E_1'$ and all other quantities do not change.
\end{theorem}

